NeST: Neural Stress Tensor Tomography by leveraging 3D Photoelasticity

Photoelasticity enables full-field stress analysis in transparent objects through stress-induced birefringence. Existing techniques are limited to 2D slices and require destructively slicing the object. Recovering the internal 3D stress distribution of the entire object is challenging as it involves solving a tensor tomography problem and handling phase wrapping ambiguities. We introduce NeST, an analysis-by-synthesis approach for reconstructing 3D stress tensor fields as neural implicit representations from polarization measurements. Our key insight is to jointly handle phase unwrapping and tensor tomography using a differentiable forward model based on Jones calculus. Our non-linear model faithfully matches real captures, unlike prior linear approximations. We develop an experimental multi-axis polariscope setup to capture 3D photoelasticity and experimentally demonstrate that NeST reconstructs the internal stress distribution for objects with varying shape and force conditions. Additionally, we showcase novel applications in stress analysis, such as visualizing photoelastic fringes by virtually slicing the object and viewing photoelastic fringes from unseen viewpoints. NeST paves the way for scalable non-destructive 3D photoelastic analysis.

==> sections/old/s4_fwd_model_v1.tex <==
\section{Photoelastic Image Formation Model}

Here we formulate polarimetric light transport through objects under mechanical stress and demonstrate by the means of a simple example how polarimetric light transport can be used to extract the underlying 3D stress distribution.
\subsection{General Case}
Consider a transparent object of arbitrary shape subject to external mechanical forces. These forces would result in a 3-dimensional distribution of the stress tensor throughout the body of the object. In this section, we derive how this 3D stress distribution alters the polarization of the state of an arbitrary ray of light passing through this object. 
\paragraph{Stress-induced birefringence}
Consider a light ray with origin $\mathbf{o}$ and direction $\mathbf{d}$ propagating with Jones vector $\mathbf{E}$ before it interacts with the transparent object at a point $\mathbf{o} + t\mathbf{d}$. Consider the plane orthogonal to the ray is spanned by two orthogonal vectors, $\mathbf{v}_0$ and $\mathbf{v}_0$. From the theory of integrated photoelasticity \cite{aben1979integrated}, change in the Jones vector upon interacting with the material is a function of the stress tensor distribution $\mathbf{S}$ of the object at that point. 
\begin{equation}
    \frac{d\mathbf{E}}{dz} = G\mathbf{E} \;,
    \label{eq:diff_stress_optic}
\end{equation}
with
\begin{equation}
G = -\frac{i}{2\pi\lambda} C \begin{bmatrix} \frac{1}{2} (\sigma'_{11} - \sigma'_{22}) & \sigma'_{12} \\ \sigma'_{12} & -\frac{1}{2} (\sigma'_{11} - \sigma'_{22}) \end{bmatrix} 
\end{equation}
Here, \(\sigma'_{ij}\) are the secondary stresses, i.e., the stresses in the plane perpendicular to the propagation vector of the light wave. We obtain \(\sigma'\) by projecting the 3D stress tensor \(S\) on that plane, spanned by two orthonormal vectors \(v_0\) and \(v_1\).
\begin{equation}
   \sigma' = \begin{pmatrix} v^T_0\mathbf{S}v_0 & v^T_0\mathbf{S}v_1 \\ v^T_1\mathbf{S}v_0 & v^T_1\mathbf{S}v_1 \end{pmatrix} . 
\end{equation}
As the ray passes through the object, we can solve for the Jones vector exiting the object as a function of the stress tensor $\mathbf{S}$, by solving Eq.~\ref{eq:diff_stress_optic}

\subsection{2D Photoelasticity}
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/circular_polariscope.pdf}
    \caption{Circular polariscope schematic}
    \label{fig:cir_pol}
\end{figure}

\paragraph{Assumptions.} We are assuming that the specimen is infinitely thin. So we only need to model a 2 dimensional stress profile. The specimen is placed in a medium with a similar refractive index. So we can neglect the surface refraction effects. 

\paragraph{Stress Tensor}
The state of stress at a point within a photoelastic material can be described by a stress tensor. For a two-dimensional case, this can be written as:

\begin{equation}
\mathbf{S} = \begin{bmatrix}
\sigma & \tau \\
\tau & -\sigma \\
\end{bmatrix}
\end{equation}

where \( \sigma \) is the normal stress and \( \tau \) is the shear stress.

\paragraph{Jones Matrix}
The stress tensor can be used to derive the Jones matrix of the material, which describes the phase shifts introduced by the material on a plane wave of light passing through it. We can write the Jones matrix as:

\begin{align}
\mathbf{J} &= \exp\left(\frac{-iCh}{\lambda} \mathbf{S}\right) \\
&= 
\begin{bmatrix}
\cos\left(\frac{\delta}{2}\right) - i\sin\left(\frac{\delta}{2}\right)\cos(2\theta) & -i\sin\left(\frac{\delta}{2}\right)\sin(2\theta) \\
-i\sin\left(\frac{\delta}{2}\right)\sin(2\theta) & \cos\left(\frac{\delta}{2}\right) + i\sin\left(\frac{\delta}{2}\right)\cos(2\theta)
\end{bmatrix}
\end{align}

where \(C\) is the material's photoelastic constant, \(h\) is the material's thickness, \(\lambda\) is the wavelength of light, \(\delta = \frac{Ch}{\lambda}\sqrt{\sigma^2 + \tau^2}\) is the phase difference between the fast and slow rays, and \(\theta = -\frac{1}{2}\arctan\left(\frac{\tau}{\sigma}\right)\) is the angle between the fast axis and the \(x\)-axis.

\paragraph{Mueller Matrix}
The Jones matrix can be transformed into a Mueller matrix using the following transformation:

\begin{equation}
\mathbf{M} = \mathbf{A} \left( \mathbf{J} \otimes \mathbf{J}^* \right)\mathbf{A}^{-1}
\end{equation}

where \(\otimes\) denotes the Kronecker product, \(\mathbf{J}^*\) is the complex conjugate of the Jones matrix, and \(\mathbf{A}\) is a transformation matrix defined as:

\begin{equation}
\mathbf{A} = \begin{bmatrix}
1 & 0 & 0 & 1 \\
1 & 0 & 0 & -1 \\
0 & 1 & 1 & 0 \\
0 & i & -i & 0
\end{bmatrix}
\end{equation}

\paragraph{Intensity Calculation}

The intensity of light captured in a polariscope can be computed as a function of the Mueller matrix and the rotation angles of the polarizers and the quarter-wave plates. 

The Mueller matrix for a linear polarizer with a transmission axis at an angle \(\alpha\) is given by:

\begin{equation}
\mathbf{P}_{\alpha} = \begin{bmatrix}
1 & \cos(2\alpha) & \sin(2\alpha) & 0 \\
\cos(2\alpha) & \cos^2(2\alpha) & \cos(2\alpha)\sin(2\alpha) & 0 \\
\sin(2\alpha) & \cos(2\alpha)\sin(2\alpha) & \sin^2(2\alpha) & 0 \\
0 & 0 & 0 & 0 \\
\end{bmatrix}
\end{equation}

The Mueller matrix for a quarter-wave plate with a fast axis at an angle \(\xi\) is given by:

\begin{equation}
\mathbf{Q}_{\xi} = \begin{bmatrix}
1 & 0 & 0 & 0 \\
0 & \cos(4\xi) & \sin(4\xi) & 0 \\
0 & -\sin(4\xi) & \cos(4\xi) & 0 \\
0 & 0 & 0 & \cos(2\xi)
\end{bmatrix}
\end{equation}

The intensity is then given by:

\begin{equation}
I = \mathbf{P}_{\beta} \mathbf{Q}_{\eta} \mathbf{M} \mathbf{Q}_{\xi} \mathbf{P}_{\alpha}[0,0]
\end{equation}

where \(\mathbf{P}_{\alpha}\) and \(\mathbf{P}_{\beta}\) are the Mueller matrices for the polarizers at angles \(\alpha\) and \(\beta\), and \(\mathbf{Q}_{\xi}\) and \(\mathbf{Q}_{\eta}\) are the Mueller matrices for the quarter-wave plates at angles \(\xi\) and \(\eta\).

\paragraph{Captured Measurements}
Here we present a table of 10 measurements taken with different angles for the polariscope, and the corresponding expressions for the intensity.

\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
\(\alpha\) & \(\xi\) & \(\eta\) & \(\beta\) & Intensity Expression \\
\hline
\(\pi/2\) & - & - & 0 & \(\sin^2\left(\frac{\delta}{2}\right) \sin^2(2\theta)\) \\
5\(\pi/8\) & - & - & \(\pi/8\) & \(\frac{1}{2}\sin^2\left(\frac{\delta}{2}\right) \left(1-\sin(4\theta)\right)\) \\
3\(\pi/4\) & - & - & \(\pi/4\) & \(\sin^2\left(\frac{\delta}{2}\right) \cos^2(2\theta)\) \\
7\(\pi/8\) & - & - & 3\(\pi/8\) & \(\frac{1}{2}\sin^2\left(\frac{\delta}{2}\right) \left(1+\sin(4\theta)\right)\) \\
\(\pi/2\) & 3\(\pi/4\) & \(\pi/4\) & \(\pi/2\) & \(\frac{1}{2} \left(1 + \cos(\delta)\right)\) \\
\(\pi/2\) & 3\(\pi/4\) & \(\pi/4\) & 0 & \(\frac{1}{2} \left(1 - \cos(\delta)\right)\) \\
\(\pi/2\) & 3\(\pi/4\) & 0 & 0 & \(\frac{1}{2} \left(1 - \sin(2\theta) \sin(\delta)\right)\) \\
\(\pi/2\) & 3\(\pi/4\) & \(\pi/4\) & \(\pi/4\) & \(\frac{1}{2} \left(1 + \cos(2\theta) \sin(\delta)\right)\) \\
\(\pi/2\) & \(\pi/4\) & 0 & 0 & \(\frac{1}{2} \left(1 + \sin(2\theta) \sin(\delta)\right)\) \\
\(\pi/2\) & \(\pi/4\) & 3\(\pi/4\) & \(\pi/4\) & \(\frac{1}{2} \left(1 - \cos(2\theta) \sin(\delta)\right)\) \\
\hline
\end{tabular}
\end{center}

\paragraph{Estimating Stress from Measurements}

From the intensity measurements, we can estimate the isochromatic parameter \(\delta\) and the isoclinic parameter \(\theta\). These are given by:

\begin{equation}
\theta_c = \frac{1}{4} \arctan \left( \frac{I_4 - I_2}{I_3 - I_1} \right)
\end{equation}

and 

\begin{equation}
\delta_c = \arctan \left( \frac{(I_9 - I_7)\sin(2\theta_c) + (I_8 - I_{10})\cos(2\theta_c)}{I_5 - I_6} \right)
\end{equation}

where \(I_1, I_2, \ldots, I_{10}\) are the intensity measurements.

With the estimated values of \(\theta\) and \(\delta\), we can then estimate the stress tensor \(\sigma\):

\begin{equation}
\mathbf{\sigma}_c = \frac{i\delta_c}{2} \begin{bmatrix}
- \cos(2\theta_c) & \sin(2\theta_c) \\
\sin(2\theta_c) &   \cos(2\theta_c)
\end{bmatrix}
\end{equation}

By fitting the measured intensities to the model intensities given by the stress tensor, we can estimate the stress distribution within the material. This process can be repeated for multiple sets of measurements to get a more accurate estimate of the stress distribution.

\subsection{Toy case: Thin disk under diametral compression}
To illustrate the dependence of polarized light transport on underlying stress, consider the case of a transparent thin circular disk compressed by equal and opposite forces applied diametrically. 
\paragraph{Stress Profile}
For this case, the stress profile is analytically given as \cite{fandino2018fringe,magalhaes2015numerical},
which define its rectangular stress components \(\sigma_x\), \(\sigma_y\), and shear stresses \(\tau_{xy}\):

\begin{equation}
\sigma_x = -\frac{2L}{\pi h} \left( \frac{x^2(R - y)}{(R - y)^2 + x^2}^2 + \frac{x^2(R + y)}{(R + y)^2 + x^2}^2 - \frac{1}{2R} \right) 
\end{equation}

\begin{equation}
\sigma_y = -\frac{2L}{\pi h} \left( \frac{(R - y)^3}{(R - y)^2 + x^2}^2 + \frac{(R + y)^3}{(R + y)^2 + x^2}^2 - \frac{1}{2R} \right) 
\end{equation}

\begin{equation}
\tau_{xy} = \frac{2L}{\pi h} \left( \frac{x(R - y)^2}{(R - y)^2 + x^2}^2 - \frac{x(R + y)^2}{(R + y)^2 + x^2}^2 \right) 
\end{equation}

In these equations, \(x\) and \(y\) refer to Cartesian coordinates in the disk domain; \(h\) and \(R\) are the thickness and radius, respectively, and \(L\) is the applied load.

% \paragraph{Stress-optic law}
% The rectangular stress components are used to calculate the principal stress components \(\sigma_1\), \(\sigma_2\), and its orientations \(\theta\), according to Eqs. (4) and (5), respectively:

% \begin{equation}
% \sigma_{1,2} = \frac{\sigma_x + \sigma_y}{2} \pm \sqrt{\left(\frac{\sigma_x - \sigma_y}{2}\right)^2 + \tau_{xy}^2} \tag{4}
% \end{equation}

% \begin{equation}
% \theta = -\frac{1}{2} \tan^{-1}\left(\frac{2\tau_{xy}}{\sigma_x - \sigma_y}\right) \tag{5}
% \end{equation}

% From the principal stresses, the stress-optic law provides Eq. (6) to calculate the isochromatic parameter \(\delta\):

% \begin{equation}
% \delta = \frac{(\sigma_1 - \sigma_2)2\pi hc}{\lambda} = C(\sigma_1 - \sigma_2)h \tag{6}
% \end{equation}

% Here, \(\lambda\) is the wavelength of the light, \(c\) is the relative optic-stress coefficient of the model, and \(C = \frac{2\pi c}{\lambda}\) is the stress-optic coefficient.

\subsection{3D Integrated Photoelasticity}

Consider a polariscope with the quarter wave plates and the output polariser or analyser at arbitrary orientations, as shown in Fig. 1. The input of unpolarised light from the source has a Stokes vector, $S$, where 

\begin{equation} 
S = [a, 0, 0, 0]^T
\end{equation}

The Mneller matrix of an ideal linear polariser whose principal axis subtends an angle $\psi$ with the vertical reference axis is 

\begin{equation}
P_{\psi} = \frac{1}{2}\begin{bmatrix}
1 & \cos 2\psi & \sin 2\psi & 0 \\ 
\cos 2\psi & \cos^2 2\psi & \cos 2\psi \sin 2\psi & 0\\
\sin 2\psi & \cos 2\psi \sin 2\psi & \sin^2 2\psi & 0 \\
0 & 0 & 0 & 0
\end{bmatrix}
\end{equation}

The Mueller matrix of a quarter wave plate with its fast axis at an angle $\phi$ to the reference axis is given by

\begin{equation}
Q_{\phi} = \begin{bmatrix}
1 & 0 & 0 & 0\\ 
0 & \cos^2 2\phi & \cos 2\phi \sin 2\phi & -\sin 2\phi\\
0 & \cos 2\phi \sin 2\phi & \sin^2 2\phi & \cos 2\phi\\
0 & \sin 2\phi & -\cos 2\phi & 0
\end{bmatrix}
\end{equation}

The three-dimensional specimen is optically equivalent to a linear retarder of retardation, $\delta$, with its fast-axis at an angle $\theta$ to the reference axis and a rotator, $\chi$. The Mueller matrix for the linear retarder is given by

\begin{equation}
M_R(\delta) = \begin{bmatrix}
1 & 0 & 0 & 0\\
0 & \cos^2 2\theta + \sin^2 2\theta \cos \delta & (1 - \cos\delta) \sin 2\theta \cos 2\theta & -\sin 2\theta \sin \delta\\ 
0 & (1 - \cos\delta) \sin 2\theta \cos 2\theta & \sin^2 2\theta + \cos^2 2\theta \cos \delta & \cos 2\theta \sin \delta\\
0 & -\sin 2\theta \sin \delta & \cos 2\theta \sin \delta & \cos \delta
\end{bmatrix}
\end{equation}

and for the rotator the matrix is

\begin{equation}
R_{\chi} = \begin{bmatrix}
1 & 0 & 0 & 0\\
0 & \cos 2\chi & -\sin 2\chi & 0\\
0 & \sin 2\chi & \cos 2\chi & 0\\  
0 & 0 & 0 & 1
\end{bmatrix}
\end{equation}

Hence the resulting Stokes vector, $S_{out}$, of the light at the output of the polariscope is obtained from

\begin{equation}
S_{out} = P_{\beta}Q_{\gamma}R_{\chi}M_R(\delta)Q_{\alpha}P_{\omega}S
\end{equation}

Thus for the orientations of the input and output elements of the polariscope given in Table 1, the intensities observed are

\begin{align}
I_1 &= \frac{a^2}{2}(1 + \sin\delta\cos2(\theta + \chi))\\
I_2 &= \frac{a^2}{2}(1 - \sin\delta\sin^2(\theta + \chi))\\  
I_3 &= \frac{a^2}{2}(1 + \sin\delta\sin^2(\theta + \chi))\\
I_4 &= \frac{a^2}{2}(1 + \cos\delta)\\
I_5 &= \frac{a^2}{2}(1 + \sin2\theta\sin\delta)\\
I_6 &= \frac{a^2}{2}(1 - \cos2\theta\cos2(\theta + \chi) - \sin2\theta\sin2(\theta + \chi)\cos\delta)
\end{align}

where $a$ is a constant of proportionality.

By combining these six phase-stepped images the characteristic parameters may be solved as 

\begin{align}
\theta + \chi &= \frac{1}{2}\tan^{-1}\frac{I_3 - I_2}{I_3 + I_2 - 2I_1}\\
\delta &= \tan^{-1}\frac{\sin2(\theta + \chi)}{2I_2 + 2I_3 - I_4 - I_3 + I_2}\sin\delta\\
\theta &= \frac{1}{2}\tan^{-1}\frac{\sin2\theta(1 - \cos2(\theta + \chi))}{\sin(\theta + \chi)\sin2\theta\cos\delta}  
\end{align}

where 

\begin{equation}
\sin2\theta = \frac{2I_5}{I_2 + I_3} - 1
\end{equation}

It can be seen from these expressions that it is theoretically possible to obtain all three characteristic parameters with only five phase-stepped images, $I_1$ to $I_5$. However, the solutions of Eqs (8)-(10) are maps of periodic parameters which need to be converted into continuous maps using unwrapping algorithms. The algorithms described by Wang and Patterson [16] use the arctangent function, from which it is straightforward to identify turning points in the data maps. If only five images were used an arc-cosine function would be required from which it is not easy to identify these turning points. Therefore it was decided to implement these algorithms with six images. 







==> sections/old/s4_fwd_model_v2.tex <==
\section{Photoelastic Image Formation Model}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/circular_polariscope.pdf}
    \caption{Our acquisition }
    \label{fig:cir_pol}
\end{figure}
In this section, we derive how the underlying three-dimensional stress distribution within a transparent object can be captured in the polarimetric light transport through the object. We demonstrate how stress present at a certain point within the object induces birefringence that we model through Jones calculus. Then we present a Monte-carlo based volume rendering approach to integrate the stress-birefringence effects into a combined Jones matrix that we can measure with a circular polariscope-based capture setup. 

\subsection{Stress Tensor Field}
Consider a transparent object of arbitrary shape subject to external mechanical forces. These external forces would result in a three-dimensional distribution of body forces throughout the body of the object modelled as mechanical stress. 

The stress at a point $\mathbf{p}$ in the material is commonly represented by the second-order cartesian stress tensor \cite{dally1978experimental}. Considering a small axis-aligned cubic element at the point $\mathbf{p}$. The stress tensor characterizes the forces on each face of this cube projected along the $x$, $y$ and $z$ axis.  The stress tensor, $S$, can be expressed as a matrix with rows as the $x$, $y$, $z$, normal directions of the faces and columns as the forces along $x$, $y$, $z$ directions each face.
\begin{equation}
\mathbf{S}(\mathbf{p}) = 
\begin{bmatrix}
\sigma_{xx} & \sigma_{xy} & \sigma_{xz} \\
\sigma_{yx} & \sigma_{yy} & \sigma_{yz} \\
\sigma_{zx} & \sigma_{zy} & \sigma_{zz}
\end{bmatrix}
\end{equation} 

Under the conditions of equillibrium $\sigma_{ij} = \sigma_{ji}$. Thus at each point, the stress tensor can be expressed as a symmetric matrix with six unkowns:
\begin{equation}
\mathbf{S}(\mathbf{p}) = 
\begin{bmatrix}
\sigma_{xx} & \sigma_{xy} & \sigma_{xz} \\
\sigma_{xy} & \sigma_{yy} & \sigma_{yz} \\
\sigma_{zx} & \sigma_{yz} & \sigma_{zz}
\end{bmatrix}
\end{equation}

\subsection{Stress-induced Birefringence}
\ad{Currently this section assumes thin hollow object and neglects refraction effects. }
\wh{I think it will be difficuylt to come up with a common notation for the full refractive case with surface boundaries. I think we can jus tstate that this is for regions of space without discontinuities; at boundaries, you get splitting of rays into relfected and refracted paths, and then things get messy. Then we cna just apply the Jones matrix for the surface interactions explicityly in the ray tracer.}
Consider a ray with origin $\mathbf{o}$ and direction $\mathbf{d}$ propagating through the transparent object under stress. The points along the ray, $\mathbf{p}(t)$ are parametrized as:
\begin{equation}
    \mathbf{p}(t) = \mathbf{o} + t\mathbf{d}
\end{equation}. We will parametrize the Jones vector and stress vector at point $\mathbf{p}(t)$ on the ray as $\mathbf{E}(t)$ and $\mathbf{S}(t)$ respectively.

Consider the plane orthogonal to the ray $(\mathbf{o}, \mathbf{d})$ is spanned by two orthogonal vectors, $\mathbf{u}$ and $\mathbf{v}$. We will define the projection of the stress tensor $\mathbf{S}$, along the orthogonal plane with $\mathbf{u} - \mathbf{v}$ axes, as the (symmetric) matrix $\mathbf{S}'$ 
\begin{equation}
   \mathbf{S}' = \begin{bmatrix} \mathbf{u}^T \mathbf{S}\mathbf{v} & \mathbf{u}^T\mathbf{S}\mathbf{v} \\ \mathbf{u}^T\mathbf{S}\mathbf{v} & \mathbf{u}^T\mathbf{S}\mathbf{v} \end{bmatrix} 
   \triangleq \begin{bmatrix}
      s'_{11} & s'_{12} \\
      s'_{12} & s'_{22} 
   \end{bmatrix}.  
\end{equation}

From the theory of integrated photoelasticity \cite{aben1979integrated}, under weak-birefringence, the change in the Jones vector upon interacting with the material is a function of the projected stress tensor distribution $\mathbf{S}'$ of the object at that point. 
\begin{equation}
    \frac{d\mathbf{E}(t)}{dt} = \mathbf{G}(t)\mathbf{E}(t) \;,
    \label{eq:diff_stress_optic}
\end{equation}
with
\begin{equation}
G = -\frac{i 2\pi C}{\lambda} \begin{bmatrix} \frac{1}{2} \left(s'_{11}(t) - s'_{22}(t)\right) & s'_{12}(t) \\ s'_{12}(t) & -\frac{1}{2} \left(s'_{11}(t) - s'_{22}(t)\right) \end{bmatrix} 
\end{equation}
where $C$ is stress-optic coefficient and $\lambda$ is the wavelength. 

We define \(\sigma\) and \(\tau\) as,
\begin{align}
\sigma(t) &= \frac{1}{2}\left(s'_{11}(t) - s'_{22}(t)\right) \\
\tau(t) &= s'_{12}(t).
\end{align}

Thus the stress optic relation can be written as

\begin{equation}
\frac{dE(t)}{dt} = -i \frac{2\pi C}{\lambda}
\begin{bmatrix}
\sigma(t) & \tau(t) \\
\tau(t) & -\sigma(t)
\end{bmatrix}
E(t)
\end{equation}

% Define matrix \(G\) as

% \begin{equation}
% G(t) = 
% \begin{bmatrix}
% \sigma(t) & \tau(t) \\
% -\tau(t) & -\sigma(t)
% \end{bmatrix}
% \end{equation}

% \begin{equation}
% \frac{dE(t)}{dt} = -i \frac{2\pi c}{\lambda} G(t) E(t)
% \end{equation}
Given the Jones vector of the ray before interacting with the object, this differential equation can be solved as an initial value problem. Bu{\ss}ler et al. \cite{bussler2015photoelasticity} use fourth order Runge-Kutta algorithm to solve the above equation and obtain net Jones matrix along the ray.  


\subsection{Approximation using Monte-Carlo Ray Marching}
\wh{This is just Euler integration, right? It seems strange to refer to 4th order RUnge Kutta above but then explain in detail the simpler Euler integration without mentioning its name}
Consider samples \( t_i \) along the ray \( j = 1, 2, \ldots, N \). Assuming \( G \) is constant between the samples \( t_i \) and \( t_{i+1} \), we have:
\begin{equation}
\frac{dE(t)}{dt} = -i \frac{2\pi C}{\lambda} G(t_i)E(t)
\end{equation}

\begin{equation}
\int_{t_i}^{t_{i+1}} \frac{dE(t)}{E(t)} = -i \frac{2\pi c}{\lambda} G(t_i) \int_{t_i}^{t_{i+1}} dt
\end{equation}

\begin{equation}
\ln \left( \frac{E(t_{i+1})}{E(t_i)} \right) = -i \frac{2\pi c}{\lambda} G(t_i) \Delta t_i
\end{equation}
where \( \Delta t_i = t_{i+1} - t_i \).

\begin{equation}
E(t_{i+1}) = \text{Exp} \left[ -i \frac{2\pi C}{\lambda} G(t_i) \Delta t_i \right] E(t_i)
\end{equation}
where Exp is complex matrix exponential.

For the entire ray we have:
\begin{equation}
E(t_N) = \prod_{i=1}^{N} \text{Exp} \left[ -i \frac{2\pi C}{\lambda} G(t_i) \Delta t_i \right] E(t_0)
\end{equation}

Thus Jones matrix along the ray \( j \) to \( j+d \) is:
\begin{equation}
J_{0,d} = \prod_{i=1}^{N} \text{Exp} \left[ -i \frac{2\pi C}{\lambda} G(t_i) \Delta t_i \right]
\end{equation}

As \( G(t_i) \) is trace-free and symmetric we have: \ad{This is a first order approximation. Correcting the derivation in appendix B to explain this}
\begin{equation}
J_{\text{net}} = \text{Exp} \left[ -i \frac{2\pi C}{\lambda} \sum_{i=1}^{N} G(t_i) \Delta t_i \right]
\end{equation}

We denote the combined matrix \( G_{\text{net}} \) as:
\begin{equation}
G_{\text{net}} = \sum_{i=1}^{N} G(t_i) \Delta t_i = 
\begin{bmatrix}
\sigma_{\text{net}} & \tau_{\text{net}} \\
\tau_{\text{net}} & -\sigma_{\text{net}}
\end{bmatrix}
\end{equation}

Where
\begin{equation}
\sigma_{\text{net}} = \sum_{i=1}^{N} \sigma_i \Delta t_i
\end{equation}
\begin{equation}
\tau_{\text{net}} = \sum_{i=1}^{N} \tau_i \Delta t_i
\end{equation}

\begin{equation}
J_{\text{net}} = \text{Exp}\left[ -i \frac{2\pi C}{\lambda} G_{\text{net}} \right]
\end{equation}

In appendix, we show this can be simplified as
\begin{equation}
J_{\text{net}} = \cos \left( -\frac{2\pi C}{\lambda} \sqrt{\sigma_{\text{net}}^2 + \tau_{\text{net}}^2} \right) \mathbf{I} 
+ j \frac{\sin \left( -\frac{2\pi C}{\lambda} \sqrt{\sigma_{\text{net}}^2 + \tau_{\text{net}}^2} \right)}{\sqrt{\sigma_{\text{net}}^2 + \tau_{\text{net}}^2}} G_{\text{net}}
\end{equation}

We define the parameters $\delta$ and $\theta$ that are termed in the photoelastic literature as isochromatic and isoclinic parameters \cite{ramesh2021developments}.
\begin{equation}
\delta = -\frac{4\pi C}{\lambda} \sqrt{\sigma_{\text{net}}^2 + \tau_{\text{net}}^2}
\label{eq:delta}
\end{equation}
\begin{equation}
2\theta = \tan^{-1} \left( \frac{\sigma_{\text{net}}}{\tau_{\text{net}}} \right)
\label{eq:theta}
\end{equation}

\begin{equation}
J_{\text{net}} = \cos \delta \mathbf{I} + j \sin \delta
\begin{bmatrix}
\cos \theta & \sin \theta \\
\sin \theta & -\cos \theta
\end{bmatrix}
\label{eq:J_net}
\end{equation}

\subsection{Captured Polarized Measurements}
We consider a circular polariscope-based setup (Fig.~\ref{fig:cir_pol}) to capture the stress-induced birefringence, derived as Jones matrix in Eq.~\ref{eq:J_net}. Light emitted by an area light source passes through a linear polarizer (LP1) with the polarization axis oriented at an angle $\alpha$ with respect to the horizontal. The linearly polarized light then passes through a quarter wave plate (QWP1) with slow axis oriented at an angle $\xi$ with respect to the horizontal. The resulting circularly polarized light passes the transparent specimen under stress. The light ray coming out of the specimen is passed through another quarter wave plate (QWP2) with slow axis oriented at an angle $\eta$ and another linear polarizer (LP2) with the polarization axis oriented at an angle $\beta$.

LP1 is fixed at a orientation $\alpha = 90^\circ$ and QWP 1 is fixed at an orientation $\xi=45^\circ$. QWP2 and LP2 are rotated to obtain multiple measurements as common in the phase shifted technique common in two-dimensional photoelasticity \cite{ramesh2021developments}. The intensity measured along the ray $I$ depends on the aggregated stress parameters $\delta$ (Eq.~\ref{eq:delta}) and $\theta$(Eq.~\ref{eq:theta}) as,

\begin{equation}
I = {I_b} + {I_a} \left[ \sin 2(\beta - \eta) \cos \delta - \sin 2(\theta - \beta) \cos 2(\beta - \eta) \sin \delta \right]
\end{equation}
, where $I_b$ is the unpolarized background intensity and $I_a$ is the intensity emitted by the area source.  Please refer to the appendix for the derivation.

We consider the size-step phase shifting technique \cite{patterson1991towards} where six measurements are obtained with varying orientations of LP2 and QWP2. The expressions for the obtained intensity are shown in Table~\ref{table:intensity_expressions}.
\input{tables/captured_measurements}

The latter four equations can be combined as shown below to yield the isoclinic parameter, $\theta$

\begin{equation}
\theta = \frac{1}{2} \arctan \left( \frac{I_5 - I_3}{I_4 - I_6} \right) 
\end{equation}

The obtained $\theta$ value can then be used to estimate the isochromatic parameters $\delta$,

\begin{equation}
\delta = \arctan \left( \frac{I_4 - I_6}{(I_1 - I_2) \cos 2\theta} \right) = \arctan \left( \frac{I_5 - I_3}{(I_1 - I_2) \sin 2\theta} \right)
\end{equation}



==> sections/old/s4_fwd_model_v3.tex <==
\section{Photoelastic Image Formation Model}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/f1_formulation_and_approach/forward_model_overview_V2.pdf}
    \caption{\textbf{Image formation model.} We develop forward model to render stress-induced birefringence from the stress field distribution in a 3D transparent object (a). In a polariscope-based setup (b), we formulate how for a ray passing through the object, the effective Jones matrix is a projection of stress tensors at points along the ray. In (c), we visualize the captured measurements for different orientations of the polariscope elements and different 3D rotations of the object. }
    \label{fig:cir_pol}
\end{figure*}
In this section, we derive how the polarimetric light transport through a transparent object encodes the underlying three-dimensional stress tensor distribution within the transparent object. We demonstrate how stress present at a certain point within the object induces birefringence that we model through Jones calculus. Then we present a Monte-Carlo based volume rendering approach to integrate the stress-birefringence effects into a combined Jones matrix that we can measure with a circular polariscope-based capture setup. 

\subsection{Stress-induced Birefringence}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/f1_formulation_and_approach/stress_tensor_v2.pdf}
    \caption{\textbf{Modeling stress induced birefringence}}
    \label{fig:projected_stress_tensor}
\end{figure*}
% \ad{Currently this section assumes thin hollow object and neglects refraction effects. } To be fixed in 4.3
% \wh{I think it will be difficuylt to come up with a common notation for the full refractive case with surface boundaries. I think we can just state that this is for regions of space without discontinuities; at boundaries, you get splitting of rays into relfected and refracted paths, and then things get messy. Then we cna just apply the Jones matrix for the surface interactions explicityly in the ray tracer.} To be fixed in 4.3
Consider a ray with origin $\mathbf{o}$ and direction $\mathbf{d}$ propagating through the transparent object under stress. The points along the ray within the object $\mathbf{p}(t)$ are parametrized as:
\begin{equation}
    \mathbf{p}(t) = \mathbf{o} + t\mathbf{d} \quad t \in [ t_n, t_f] \;.
\end{equation} 
We denote the Jones vector and the stress tensor at point $\mathbf{p}(t)$ on the ray as $\mathbf{E}(t)$ and $\mathbf{S}(t)$ respectively.

\paragraph{Projected stress}
Consider the plane orthogonal to the ray $(\mathbf{o}, \mathbf{d})$ is spanned by two orthonormal basis vectors, $\mathbf{u}$ and $\mathbf{v}$. We will define the projection of the stress tensor $\mathbf{S}(t)$, along the orthogonal plane with $\mathbf{u} - \mathbf{v}$ axes, as the symmetric matrix $\mathbf{S}'(t)$ 
\begin{equation}
   \mathbf{S}'(t) = \begin{bmatrix} \mathbf{u}^T \mathbf{S}(t)\mathbf{v} & \mathbf{u}^T\mathbf{S}(t)\mathbf{v} \\ \mathbf{u}^T\mathbf{S}(t)\mathbf{v} & \mathbf{u}^T\mathbf{S}(t)\mathbf{v} \end{bmatrix} 
   \triangleq \begin{bmatrix}
      \sigma_{\mathbf{u}\mathbf{v}} & \sigma_{\mathbf{u}\mathbf{v}} \\
      \sigma_{\mathbf{uv}} & \sigma_{\mathbf{vv}}
   \end{bmatrix} \; . 
   \label{eq:projected_stress}
\end{equation}
\paragraph{Stress-optic relation}
This projected stress tensor $\mathbf{S}'(t)$ induces a weak birefringence along the ray at $\mathbf{p}(t)$ \cite{aben1979integrated}. This birefringence effect can be modeled as the change in the Jones vector at that point through the stress-optic relation
\begin{equation}
    \frac{d\mathbf{E}(t)}{dt} = \mathbf{G}(t)\mathbf{E}(t) \;,
    \label{eq:diff_stress_optic}
\end{equation}
where $\mathbf{G}(t)$ depends on the projected stress as
\begin{equation}
\mathbf{G}(t) = -\frac{i 2\pi C}{\lambda} \begin{bmatrix} \frac{1}{2} \left(s'_{11}(t) - s'_{22}(t)\right) & s'_{12}(t) \\ s'_{12}(t) & -\frac{1}{2} \left(s'_{11}(t) - s'_{22}(t)\right) \end{bmatrix} .
\end{equation}
Here $C$ is the stress-optic coefficient that depends on the material properties of the object and $\lambda$ is the wavelength of light. 

By defining
$\sigma(t) = \frac{1}{2}\left(s'_{11}(t) - s'_{22}(t)\right)$ and $\tau(t) = s'_{12}(t)$ we can denote $\mathbf{G}(t)$ as 
\begin{align}
\mathbf{G}(t) = 
-i \frac{2\pi C}{\lambda}
\begin{bmatrix}
\sigma(t) & \tau(t) \\
\tau(t) & -\sigma(t) \;.
\end{bmatrix} \label{eq:G_sig_tau}
\end{align}
and the stress optic relation from Eq.~\ref{eq:diff_stress_optic} can be written as
\begin{equation}
\frac{dE(t)}{dt} = -i \frac{2\pi C}{\lambda}
\begin{bmatrix}
\sigma(t) & \tau(t) \\
\tau(t) & -\sigma(t) \;.
\end{bmatrix}
E(t) \label{eq:stress_optic_sig_tau}
\end{equation}
% Define matrix \(G\) as

% \begin{equation}
% G(t) = 
% \begin{bmatrix}
% \sigma(t) & \tau(t) \\
% -\tau(t) & -\sigma(t)
% \end{bmatrix}
% \end{equation}

% \begin{equation}
% \frac{dE(t)}{dt} = -i \frac{2\pi c}{\lambda} G(t) E(t)
% \end{equation}
% Given the Jones vector of the ray before interacting with the object, this differential equation can be solved as an initial value problem. Bu{\ss}ler et al. \cite{bussler2015photoelasticity} use fourth order Runge-Kutta algorithm to solve the above equation and obtain net Jones matrix along the ray.  


\subsection{Monte-Carlo Integrated Photoelasticity}
\label{sec:integrated_photoelasticity}
Integrated photoelasticity \cite{aben1979integrated} aggregates the change in Jones vector at each point along the ray from Eq.~\ref{eq:stress_optic_sig_tau} aggregated to obtain the net change of Jones vector along the ray as
\begin{equation}
    \int_{t_n}^{t_f}{\frac{d\mathbf{E}(t)}{dt}} = \int_{t_n}^{t_f}{\mathbf{G}(t)\mathbf{E}(t)} \;,
    \label{eq:integrated_stress_optic}
\end{equation}
Bu{\ss}ler et al. \cite{bussler2015photoelasticity} compute this integral as Euler integration using the 4th order Runge Kutta (RK-4) algorithm. However, this approach is not well suited for solving the inverse optimization.\ad{Need to refine this claim and ground it with a result.} Here we derive the Monte-Carlo integration formulation for integrated photoelasticity and show how Poincar\'{e}'s equivalence theorem \cite{hammer2004characteristic} simplifies the integral computation.
% Fixed \wh{This is just Euler integration, right? It seems strange to refer to 4th order RUnge Kutta above but then explain in detail the simpler Euler integration without mentioning its name}
%Fixed \textcolor{red}{AV: The definition of G seems inconsistent. Eqn 6 has the constants outside as part of G while Eqn 10 it is outside of G.}
\paragraph{Monte-Carlo Integration}
Consider samples \( t_i \) along the ray \( j = 1, 2, \ldots, N \). Assuming \( G \) is constant between the samples \( t_i \) and \( t_{i+1} \), integrated photoelasticity equation Eq. ~\ref{eq:integrated_stress_optic} between $t_i$ and $t_{i+1}$ can be approximated as

\begin{equation}
\int_{t_i}^{t_{i+1}} d\mathbf{E(t)} = \mathbf{G}(t_i) \int_{t_i}^{t_{i+1}} \mathbf{E(t)}dt
    \label{eq:integrated_stress_optic}
\end{equation}

% \begin{equation}
% \ln \left( \frac{E(t_{i+1})}{E(t_i)} \right) = -i \frac{2\pi c}{\lambda} G(t_i) \Delta t_i
% \end{equation}

\begin{equation}
\mathbf{E}(t_{i+1}) = \text{Exp}\left(\mathbf{G}(t_i) \Delta t_i \right) \mathbf{E}(t_i)
\end{equation}
where Exp is the complex matrix exponential function and  \( \Delta t_i = t_{i+1} - t_i \). We denote the transformation from $\mathbf{E}(t_i)$ to $\mathbf{E}(t_{i+1})$ as the Jones matrix $\mathbf{J}(t_i)$:
\begin{align}
    \mathbf{J}(t_i) = \text{Exp}\left(\mathbf{G}(t_i) \Delta t_i \right) 
\end{align}
We can then express this Jones matrix as a function of projected stress at $t_i$ by substituting $\mathbf{G}(t)$ from Eq.~\ref{eq:G_sig_tau}:
\begin{align}
    \mathbf{J}(t_i) = \text{Exp}\left(-i \frac{2\pi C}{\lambda}
\begin{bmatrix}
\sigma(t) & \tau(t) \\
\tau(t) & -\sigma(t) 
\end{bmatrix} \Delta t_i \right)  
\label{eq:J_G}\;.
\end{align}
In App.~\ref{app:exp_j_A}, we show that Eq.~\ref{eq:J_G} can be simplified as,
\begin{equation}
\mathbf{J}(t_i) = \cos \left( -\frac{2\pi C}{\lambda} \sqrt{\sigma_{i}^2 + \tau_{i}^2} \right) \mathbf{I} 
+ I \frac{\sin \left( -\frac{2\pi C}{\lambda} \sqrt{\sigma_{i}^2 + \tau_{i}^2} \right)}{\sqrt{\sigma_{i}^2 + \tau_{i}^2}} G_{i}
\end{equation}
where we denote $\sigma(t_i)$ and $\tau(t_i)$ as $\sigma_i$ and $t_i$ respectively.
We define the parameters $\delta_i$ and $\theta_i$ that are termed in the photoelastic literature as isochromatic and isoclinic parameters \cite{ramesh2021developments}.
\begin{align}
\delta_i = -\frac{4\pi C}{\lambda} \sqrt{\sigma_i^2 + \tau_i^2} \quad \quad 
\theta_i = \frac{1}{2} \tan^{-1} \left( \frac{\sigma_{i}}{\tau_{i}} \right)
\label{eq:delta_theta}
\end{align}
We can express the Jones matrix in terms of these parameters as,
\begin{equation}
\mathbf{J}\left(t_i\right) = \cos \delta_i/2
\begin{bmatrix}
1 & 0 \\
0 & 1
\end{bmatrix}
+ i \sin \delta_i/2
\begin{bmatrix}
\cos 2\theta_i & \sin 2\theta_i \\
\sin 2\theta_i & -\cos 2\theta_i
\end{bmatrix}
\label{eq:J_retarder} \; ,
\end{equation} 
This Jones matrix can also be understood as that of a retarder element with retardation $\delta$ oriented with slow axis making an angle $\theta$ with the `horizontal` basis vector $\textbf{u}$ \cite{collett2005field}.

Aggregating along the entire ray, we can write the final Jones vector $\mathbf{E}(t_N)$ as a series of complex matrix multiplications.
\begin{equation}
\mathbf{E}(t_N) = \left(\prod_{i=1}^{N} \mathbf{J}\left(t_i\right)\right) \mathbf{E}(t_0) \;.
\end{equation}

We denote the net Jones matrix along the ray as $\mathbf{J}_\text{net}$
\begin{equation}
\mathbf{J}_\text{net} = \prod_{i=1}^{N} \mathbf{J}(t_i) \;.
\label{eq:integrated_photoelasticity_Jones}
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/f1_formulation_and_approach/poincare_v1.pdf}
    \caption{\textbf{Modeling integrated photoelasticity}: a) By ray marching, we sample points along the queried ray. b) We model each segment between the sampled points,$t_{i}$ and $t_{i+1}$ as a retarder with retardance $\delta_i$ and slow-axis orientation $\theta_i$. c) From Poincare equivalence theorem, stack of any number of retarders is equivalent to a single retarder with parameters $(\delta_{\textit{eq}},\theta_{\textit{eq}})$ followed by a rotator with rotation $\gamma_{\mathrm{eq}}$ }
    \label{fig:equivalence_theorem}
\end{figure}
\paragraph{Employing equivalence theorem} The net Jones matrix can be understood as a combination of $N$ retarders along the ray each with a different retardance $\delta_i$ and orientation $\theta_i$. Poincare's equivalence theorem states that the polarization properties of a combination of retarders are equivalent to that of a retarder followed by a rotator. Thus, the aggregate Jones matrix $\mathbf{J}_{\text{net}}$ can be represented by the product of Jones matrix of retarder with retardance $\delta_\text{net}$ and orientation $\theta'_\text{net}$ and a rotator with $\theta_\text{net}$. In App.~\ref{app:equivalence}, we show demonstrate the equivalence theorem for Eq.~\ref{eq:integrated_photoelasticity_Jones} and show that $\mathbf{J}_{net}$ can be expressed as     
\begin{equation}
\mathbf{J}_\text{net} = 
\cos{\delta_\text{net}}
\begin{bmatrix}
\cos \gamma_\text{net} & \sin \gamma_\text{net}\\
\sin \gamma_\text{net} & -\cos \gamma_\text{net} 
\end{bmatrix} 
+ i \sin{\delta_\text{net}} 
\begin{bmatrix}
\cos \theta_\text{net} & \sin \theta_\text{net}\\
\sin \theta_\text{net} & -\cos \theta_\text{net} 
\end{bmatrix} 
\label{eq:J_net} \;,
\end{equation}
where $\theta_\text{net} = \theta'_\text{net} - \gamma_\text{net}$.


\paragraph{Linear approximation} In App.~\ref{app:first_order_approx}, we show that under first-order approximations, our formulation simplifies to a linear combination of projected stress followed by phase wrapping. Prior works leverage this approximation to formulate photoelastic tomography as linear tensor tomography \cite{szotten2011limited,sharafutdinov2012integral}. Consider the projected stress components $\sigma_{\text{lin}}$ and $\tau_{\text{lin}}$ defined as
\begin{equation}
\sigma_{\text{lin}} = \sum_{i=1}^{N} \sigma_i \Delta t_i
\quad \quad
\tau_{\text{lin}} = \sum_{i=1}^{N} \tau_i \Delta t_i
\label{eq:sig_tau_lin}
\end{equation}
In App~\ref{app:first_order_approx}, we show that the aggregated Jones matrix under first-order approximation $\mathbf{J}_{\text{lin}}$ can be written as 
\begin{equation}
\mathbf{J}_{\text{lin}} = \cos \delta_{\text{lin}}/2 \mathbf{I} + j \sin \delta_{\text{lin}}/2
\begin{bmatrix}
\cos 2\theta_{\text{lin}} & \sin 2\theta_{\text{lin}} \\
\sin 2\theta_{\text{lin}} & -\cos 2\theta_{\text{lin}}
\end{bmatrix}
\label{eq:J_approx} \;,
\end{equation}
where
\begin{align}
\delta_{\text{lin}} = -\frac{4\pi C}{\lambda} \sqrt{\sigma_{\text{lin}}^2 + \tau_{\text{lin}}^2} \quad \quad 
\theta_{\text{lin}} = \frac{1}{2} \tan^{-1} \left( \frac{\sigma_{\text{lin}}}{\tau_{\text{lin}}} \right)
\end{align}
\label{eq:delta_theta}
\paragraph{Our general formulation vs linear approximation} In the most general case, the projected stress tensor at each point is encoded as Jones matrices (Eq.~\ref{eq:J_retarder}) where there is phase wrapping of stress values due to sinusoidal expressions. Then all Jones matrices are aggregated using Jones matrix multiplication. The linear approximation employed by prior works (\cite{szotten2011limited,sharafutdinov2012integral}), first aggregates the projected stress values using Eq.~\ref{eq:sig_tau_lin} and then does phase wrapping Eq.~\ref{eq:J_approx}. 

Due to \textit{first aggregate then phase wrap}, prior works rely on first phase wrapping the projected J value and then perform linear tensor tomography. Our \textit{first phase wrap and then aggregate} enables first tomography and then phase wrapping. When solving the inverse problem of reconstructing stress from Jones matrix, we can thus perform phase unwrapping in stress space rather than in projected Jones space. Thus we can directly apply smoothness prior in stress space and obtain better reconstruction than \textit{first aggregate then phase wrap} approach \ad{Refine the claim and link result}. 

Moreover, the aggregated Jones matrix in the general case (Eq.~\ref{eq:J_net}) is parametrized by three characteristic parameters $\delta_{net}$, $\theta_{net}$ and $\gamma_{net}$. Aggregated Jones matrix in linear case (Eq.~\ref{eq:J_approx}) is modeled as an equivalent retarder with parameters $\delta_{lin}$ and $\theta_{net}$ and no rotator. Thus the linear approximation is not sufficient to model the rotation of polarization due to integrated photoelasticity.

\subsection{Captured Polariscope Measurements}
\label{sec:polariscope}
% Fixed \textcolor{red}{AV: sudden jump here. perhaps a few sentences pointing out from the previous eqna whre the tie into measurements is would make the transition smoother.}

In Sec.~\ref{sec:integrated_photoelasticity}, we showed that the Jones matrix Eq.~\ref{eq:J_net} corresponding to each ray passing through the object encodes a projection of the object's stress distribution. Here we show how we can measure this Jones matrix by emitting and detecting different polarization states of light.

\paragraph{Circular polariscope setup}
We consider a circular polariscope-based setup (Fig.~\ref{fig:cir_pol}) to capture components of the Jones matrix in Eq.~\ref{eq:J_net}. Light emitted by an area light source passes through a linear polarizer (LP1) with the polarization axis oriented at an angle $\alpha$ with respect to the horizontal. The linearly polarized light then passes through a quarter wave plate (QWP1) with fast axis oriented at an angle $\rho$ with respect to the horizontal. The resulting circularly polarized light passes the transparent specimen under stress. The light ray coming out of the specimen is passed through another quarter wave plate (QWP2) with fast axis oriented at an angle $\eta$ and another linear polarizer (LP2) with the polarization axis oriented at an angle $\beta$.

\paragraph{Captured intensity}
Consider $\mathbf{E}(\alpha)$ as the Jones vector of light emitted from the LP1 and $\mathbf{Q}(\rho)$,$\mathbf{Q}(\eta)$ and $\mathbf{L}(\beta)$ as the Jones matrices of QWP1, QWP2 and LP2 respectively. The effective Jones matrix as derived in Eq.~\ref{eq:J_net} depends on the characteristic parameters $\delta_{net}$, $\theta_{net}$ and $\gamma_{net}$.
The refraction into and outside the object also alters the polarization state based on the surface normals at those points. At the entry and exit points of the ray, $t_n$ and $t_f$, consider the Jones matrix depending on the surface normals $\mathbf{R}(t_n)$  and $\mathbf{R}(t_f)$.
Using Jones Calculus, the Jones vector of light reaching the detector $\mathbf{E}_d$is given by the complex matrix multiplication:
\begin{align}
    \mathbf{E}_{\text{cap}} = \mathbf{L}(\beta)\mathbf{Q}(\eta)\mathbf{R}(t_n)\mathbf{J}_{\text{net}}\mathbf{R}(t_f)\mathbf{Q}(\rho)\mathbf{E}(\alpha)
\end{align}
The captured intensity on the detector $I_d$ can be obtained from the Jones vector $\mathbf{E}$ by combining net intensity along orthogonal dimensions $\mathbf{u}$ and $\mathbf{v}$. 
\begin{align}
    I_\text{cap} = E_\mathbf{u}E_\mathbf{u}^* + E_\mathbf{v}E_\mathbf{v}^*
\end{align}
By varying the polariscope element angles $\alpha$, $\rho$, $\eta$ and $\beta$, we can obtain multiple intensity measurements that encode the characteristic parameters $\delta_{\text{net}}$, $\theta_{\text{net}}$ and $\gamma_{\text{net}}$.

\paragraph{Phase shifting technique}
We consider the size-step phase shifting technique \cite{patterson1991towards} that is common in 2D photoelasticity and is extended to integrated photoelasticity \cite{tomlinson2002use}. Here the refraction effects at the boundaries of the object are neglected by either placing the object in a refractive index matched liquid \cite{abrego2019experimental} or assuming thin surfaces. Six measurements are obtained with varying orientations of LP1, LP2 and QWP2. LP1 is fixed at an orientation $\alpha = 90^\circ$. The expressions for the configurations of polariscope elements and the obtained intensities are shown in Table~\ref{table:intensity_expressions} 
\input{tables/captured_measurements_3D}
\paragraph{Acquisition with polarization camera}
Conventional polariscope systems involve mechanical rotations of the polarizers and quarter wave plates on the camera and emitter. In the proposed measurement scheme, we propose leveraging the emerging snapshot polarization cameras. These cameras comprise a repeating grid of polarizer filters with four different rotation angles $\beta$ placed directly on the sensor. Snapshot polarization camera allows us to remove one mechanical rotation. Compared to conventional 6-step phase shifting orientations, we obtain 4 measurements for every rotation $\eta$ and $\rho$ resulting in more measurement diversity. Please refer to App.~\ref{app:phase_shiftin_technique}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/figure_sketches/Renderings_from_multiple_3D.png}
    \caption{Rendered images from multiple viewpoints}
    \label{fig:render_multiple_views}
\end{figure}
\paragraph{Measurements along multiple 3D rotations}
Every ray measures a $2\times2$ projection of the $3\times3$ stress tensors along that ray (Eq.~\ref{eq:projected_stress}). One orientation of the camera with respect to the object, thus provides only a low dimensional slice of the underlying 3-dimensional stress tensor distribution. By varying the relative orientation of the object by performing 3D rotations of either the object or the camera, we can obtain multiple projections of the stress tensor.
% yinput{tables/captured_16_measurements}

% The latter four equations can be combined as shown below to yield the isoclinic parameter, $\theta$

% \begin{equation}
% \theta - \gamma = \frac{1}{2} \arctan \left( \frac{I_5 - I_3}{I_4 - I_6} \right) 
% \end{equation}

% The obtained $\theta$ value can then be used to estimate the isochromatic parameters $\delta$,

% \begin{equation}
% \delta = \arctan \left( \frac{I_4 - I_6}{(I_1 - I_2) \cos 2(\theta- \gamma)} \right) 
% % = \arctan \left( \frac{I_5 - I_3}{(I_1 - I_2) \sin 2\theta} \right)
% \end{equation}


\begin{comment}
\begin{align}
\hat{\theta}-\hat{\gamma} &= 0.5 \cdot \tan^{-1}\left(\frac{I_3 - I_1}{2I_0 - I_3 - I_1}\right) \\
\hat{\delta} &= \tan^{-1}\left(\frac{I_3 - I_1}{(2I_2 - I_3 - I_1) \cdot \sin[2(\hat{\theta}-\hat{\gamma})]}\right) \\
\hat{\theta}+\hat{\gamma} &= 0.5 \cdot \tan^{-1}\left(\frac{I_3 + I_1 - 2\left(\frac{I_5}{\sin[2(\hat{\theta} + \hat{\gamma})]}\right) - \sin[2(\hat{\theta}-\hat{\gamma})]\cos(\hat{\delta})}{\cos[2(\hat{\theta}-\hat{\gamma})]}\right)^{-1}
\end{align}
, where $\sin[2(\hat{\theta} + \hat{\gamma})] = \frac{2I_4 - I_3 - I_1}{\sin(\hat{\delta})}$

From these parameters we can estimate the unique elements of Jones matrix:
\begin{align}
a &= cos(\hat{\delta})cos(2\hat{\gamma})\\
b &= sin(\hat{\delta})cos(2\hat{\gamma})\\
c &= sin(\hat{\delta})sin(2\hat{\theta})\\
d &= cos(\hat{\delta})sin(2\hat{\theta})\\
J_{\text{net}}  &= 
\begin{bmatrix}
a & d \\
d & -a 
\end{bmatrix}
+ j 
\begin{bmatrix}
b & c \\
c & -b
\end{bmatrix}
\end{align}
\end{comment}

==> sections/old/s4_fwd_model_v4.tex <==
\section{Photoelastic Image Formation Model}

In this section, we derive how the polarimetric light transport through a transparent object encodes its underlying three-dimensional stress tensor distribution. We demonstrate how stress present at a certain point within the object induces birefringence that we model through Jones calculus. Then we present a volume rendering approach to integrate the stress-birefringence effects into an equivalent Jones matrix that we can measure with a polariscope-based capture setup. 

\subsection{Stress-induced Birefringence}
\label{sec:birefringence}
Consider a ray with origin $\mathbf{o}$ and direction $\mathbf{d}$ propagating through the transparent object under stress. The points $\mathbf{p}(t)$ along the ray and within the object are parametrized as:
\begin{equation}
    \mathbf{p}(t) = \mathbf{o} + t\mathbf{d} \quad t \in [ t_n, t_f] \;.
\end{equation} 
The stress at the point $\mathbf{p}(t)$ is modeled by the Cartesian stress tensor $\mathbf{S}(t)$ (Eq.~\ref{eq:stress_tensor}). We demonstrate how, due to stress-induced birefringence, this stress tensor is encoded in the polarimetric light transport using Jones calculus. 

\paragraph{Projected stress tensor}
Consider the plane orthogonal to the ray $(\mathbf{o}, \mathbf{d})$ is spanned by two orthonormal basis vectors, $\mathbf{u}$ and $\mathbf{v}$. The projection of the $3\times 3$ stress tensor $\mathbf{S}(t)$ along the orthogonal plane with $\mathbf{u} - \mathbf{v}$ axes is denoted as the $2 \times 2$ symmetric matrix $\mathbf{S}'(t)$ 
\begin{equation}
   \mathbf{S}'(t) = \begin{bmatrix} \mathbf{u}^T \mathbf{S}(t)\mathbf{u} & \mathbf{u}^T\mathbf{S}(t)\mathbf{v} \\ \mathbf{u}^T\mathbf{S}(t)\mathbf{v} & \mathbf{v}^T\mathbf{S}(t)\mathbf{v} \end{bmatrix} 
   \triangleq \begin{bmatrix}
      \sigma_{\mathbf{uu}} & \sigma_{\mathbf{u}\mathbf{v}} \\
      \sigma_{\mathbf{uv}} & \sigma_{\mathbf{vv}}
   \end{bmatrix} \; . 
   \label{eq:projected_stress}
\end{equation}
% Fixed
% \wh{fixed r1c1 in the matrix, please double check.}
\paragraph{Principal stresses}
For general choices of the orthonormal basis $(\mathbf{u},\mathbf{v})$, $\mathbf{S}'(t)$ is a non-diagonal matrix, with the diagonal entries corresponding to the normal stress and non-diagonal entries corresponding to tangential stress. We show in App. \ref{app:principal_stress}, there exists an orthonormal basis $(\mathbf{v_1},\mathbf{v_2})$ with diagonal projected stress $\mathbf{S'}$, i.e.,
% \wh{I don't like that we have $\mathbf{u},\mathbf{v}$ for the original coordinate system and then $\mathbf{v}_1,\mathbf{v}_2$ for the rotated one. How about using a bar or tilde or prime on $\mathbf{u},\mathbf{v}$?}
\begin{equation}
 \begin{bmatrix} \mathbf{v}_1^T \mathbf{S}(t)\mathbf{v}_1 & \mathbf{v}_1^T\mathbf{S}(t)\mathbf{v}_2 \\ \mathbf{v}_1^T\mathbf{S}(t)\mathbf{v}_2 & \mathbf{v}_2^T\mathbf{S}(t)\mathbf{v}_2 \end{bmatrix} 
   \triangleq \begin{bmatrix}
      \sigma_1 & 0 \\
      0 & \sigma_2
   \end{bmatrix} \; ,
   \label{eq:principal_stress}
\end{equation}
with $\sigma_1 > \sigma_2$
Along $\mathbf{v}_1$ and $\mathbf{v}_2$ directions, there is only normal stress: $\sigma_1$ and $\sigma_2$ respectively that are termed as principal stresses. In App. \ref{app:principal_stress}, we derive that for any general $\mathbf{u},\mathbf{v}$ basis the difference of principle stresses depends on the components of $\mathbf{S}'$  as 
\begin{equation}
   \sigma_2 - \sigma_1 = \sqrt{\left(\sigma_{\mathbf{vv}} - \sigma_{\mathbf{uu}} \right)^2 + {\sigma_{\mathbf{uv}}}^2} \; .
\end{equation}
The angle $\theta$ made by the principle stress $\sigma_1$ with $\mathbf{u}$ is 
\begin{equation}
   \theta = \frac{1}{2}\tan^{-1}\left(\frac{2\sigma_{\mathbf{uv}}}{\sigma_{\mathbf{vv}}-\sigma_{\mathbf{uu}}}\right) \; . \label{eq:theta}
\end{equation}
\paragraph{Stress-optic relation}
Consider the segment of length $\Delta$ along the ray around the point $\mathbf{p}(t)$. The length $\Delta$ is small so that there is no stress variation along the segment. Assuming weak birefringence, stress-optic relation \cite{dally1978experimental} states that the phase difference $\delta(t)$ between the principal directions $(\mathbf{v_1}$,$\mathbf{v_2})$ is proportional to principal stress difference $\sigma_1 - \sigma_2$  and is given as:
\begin{equation}
    \delta(t) = \frac{2\pi \Delta C}{\lambda} \left( \sigma_2 - \sigma_1 \right),
\end{equation}
where $C$ is the stress-optic coefficient that depends on the material properties of the object and $\lambda$ is the wavelength of light.
\paragraph{Jones matrix}
Next we can model this stress-induced birefringence at the small segment around $\mathbf{p}(t)$ as a Jones matrix denoted as $\mathbf{J}(t)$. The definition of Jones matrix depends on the orthonal basis for Jones vectors. If we consider the Jones vectors are defined based on principal stress directions $(\mathbf{v_1},\mathbf{v_2})$, then the Jones matrix $\hat{\mathbf{J}}(t)$ corresponds to that of a retarder with retardance $\delta$ and slow axis along $\mathbf{v_1}$ which is given as \cite{collett2005field}, 
\begin{align}
    \hat{\mathbf{J}}(t) = \begin{bmatrix}
                            e^{i\nicefrac{\delta}{2}} & 0 \\
                            0 & e^{-i\nicefrac{\delta}{2}} \\ 
                          \end{bmatrix} \; .
\end{align}
The principal directions are not known apriori. General orthonormal basis vector $(\mathbf{u},\mathbf{v})$ is rotated $\theta$ from the principal directions $(\mathbf{v_1},\mathbf{v_2})$ as given by Eq.~\ref{eq:theta}. For the Jones vectors with orthonormal basis along $(\mathbf{u},\mathbf{v})$, the Jones matrix corresponds to that of a retarder with phase $\delta$ and orientation $\theta$ from the slow axis ($\mathbf{u}$) which is given as \cite{collett2005field}:
\begin{align}
\mathbf{J}(t) = \cos \left(\nicefrac{\delta}{2}\right)
\begin{bmatrix}
1 & 0 \\
0 & 1
\end{bmatrix}
+ i \sin \left(\nicefrac{\delta}{2}\right)
\begin{bmatrix}
\cos 2\theta & \sin 2\theta \\
\sin 2\theta & -\cos 2\theta
\end{bmatrix}
\label{eq:J_main} \; ,
\end{align}

\subsection{3D Photoelasticity}
\label{sec:integrated_photoelasticity}

\paragraph{Integrated photoelasticity using ray marching}
Consider $N$ samples along the ray parametrized as $t_i, i = 1, 2, \ldots, N$. Considering sufficiently large number of samples, we approximate the stress between the samples \( t_i \) and \( t_{i+1} \) to be constant., From Eq. ~\ref{eq:J_main}, the segment between $t_i$ and $t_{i+1}$ can then be approximated as a retarder with retardance $\delta_i$ and slow axis orientation $\theta_i$.

%%%%% Integrated photoelasticity formulation
%%%% TODO: Add to appendix
% This birefringence effect can be modeled as the change in the Jones vector at that point through the stress-optic relation
% \begin{equation}
%     \frac{d\mathbf{E}(t)}{dt} = \mathbf{G}(t)\mathbf{E}(t) \;,
%     \label{eq:diff_stress_optic}
% \end{equation}
% where $C$ is the stress-optic coefficient that depends on the material properties of the object and $\lambda$ is the wavelength of light $\mathbf{G}(t)$ is the trace-free version of the projected stress defined as :
% \begin{equation}
% \mathbf{G}(t) = -\frac{i 2\pi C}{\lambda}\left(\mathbf{S}'(t) - \mathrm{tr}(\mathbf{S}'(t))/2 I_2 \right)\;,
% \label{eq: G_def}
% \end{equation}
% where $\mathrm{tr}$ denotes trace-free operation and $I_2$ is $2\times2$ identity matrix.
% For a portion of the object between $t-\Delta$ to $t+\Delta$, omputing the change in Jones vector amounts to integrating Eq.~\ref{eq:diff_stress_optic} as:

% \begin{equation}
%     \int_{t-\Delta}^{t+\Delta}{\frac{d\mathbf{E}(t)}{dt}} = \int_{t-\Delta}^{t+\Delta}{\mathbf{G}(t)\mathbf{E}(t)} \;,
%     \label{eq:integrated_stress_optic}
% \end{equation}
% Assuming $\Delta$ is short enough so that the stress doesn't wary substantially in the material, we can approximate the integral as:

% \begin{align}
% \int_{t-\Delta}^{t+\Delta} d\mathbf{E(t)} &= \mathbf{G}(t) \int_{t-\Delta}^{t+\Delta} \mathbf{E(t)}dt \\
% \mathbf{E}(t + \Delta) &= \text{Exp}\left(\mathbf{G}(t) \Delta \right) \mathbf{E}(t - \Delta)
%     \label{eq:integrated_stress_optic}
% \end{align}
% We denote this change in Jones vector at $t$ as the Jones matrix $\mathbf{J}(t)$. Thus,
% \begin{align}
%     \mathbf{J}(t) = \mathrm{Exp}(\mathbf{G}(t)\Delta)
% \end{align}
% For the special case when the orthonormal basis $\mathbf{u},\mathbf{v}$ aligns with the principle stress directions $\mathbf{v}_1,\mathbf{v}_2$, from Eq.~\ref{eq: G_def} and Eq.~\ref{eq:principal_stress}, we have :
% \begin{align}
%    \mathbf{G}(t)  = -\frac{i 2\pi C}{\lambda}\begin{bmatrix}
%                                         (\sigma_1-\sigma_2)/2 & 0 \\
%                                         0 & -(\sigma_1 - \sigma_2)/2 \\
%                                              \end{bmatrix} \; ,
% \end{align}
% \subsection{3D Photoelasticity}
% \label{sec:integrated_photoelasticity}
% Integrated photoelasticity \cite{aben1979integrated} aggregates the change in Jones vector at each point along the ray from Eq.~\ref{eq:stress_optic_sig_tau} aggregated to obtain the net change of Jones vector along the ray as
% \begin{equation}
%     \int_{t_n}^{t_f}{\frac{d\mathbf{E}(t)}{dt}} = \int_{t_n}^{t_f}{\mathbf{G}(t)\mathbf{E}(t)} \;,
%     \label{eq:integrated_stress_optic}
% \end{equation}
% Bu{\ss}ler et al. \cite{bussler2015photoelasticity} compute this integral as Euler integration using the 4th order Runge Kutta (RK-4) algorithm. However, this approach is not well suited for solving the inverse optimization.\ad{Need to refine this claim and ground it with a result.} Here we derive the Monte-Carlo integration formulation for integrated photoelasticity and show how Poincar\'{e}'s equivalence theorem \cite{hammer2004characteristic} simplifies the integral computation.
% % Fixed \wh{This is just Euler integration, right? It seems strange to refer to 4th order RUnge Kutta above but then explain in detail the simpler Euler integration without mentioning its name}
% %Fixed \textcolor{red}{AV: The definition of G seems inconsistent. Eqn 6 has the constants outside as part of G while Eqn 10 it is outside of G.}
% \paragraph{Monte-Carlo Integration}
% Consider samples \( t_i \) along the ray \( j = 1, 2, \ldots, N \). Assuming \( G \) is constant between the samples \( t_i \) and \( t_{i+1} \), integrated photoelasticity equation Eq. ~\ref{eq:integrated_stress_optic} between $t_i$ and $t_{i+1}$ can be approximated as

% \begin{equation}
% \int_{t_i}^{t_{i+1}} d\mathbf{E(t)} = \mathbf{G}(t_i) \int_{t_i}^{t_{i+1}} \mathbf{E(t)}dt
%     \label{eq:integrated_stress_optic}
% \end{equation}

% % \begin{equation}
% % \ln \left( \frac{E(t_{i+1})}{E(t_i)} \right) = -i \frac{2\pi c}{\lambda} G(t_i) \Delta t_i
% % \end{equation}

% \begin{equation}
% \mathbf{E}(t_{i+1}) = \text{Exp}\left(\mathbf{G}(t_i) \Delta t_i \right) \mathbf{E}(t_i)
% \end{equation}
% where Exp is the complex matrix exponential function and  \( \Delta t_i = t_{i+1} - t_i \). We denote the transformation from $\mathbf{E}(t_i)$ to $\mathbf{E}(t_{i+1})$ as the Jones matrix $\mathbf{J}(t_i)$:
% \begin{align}
%     \mathbf{J}(t_i) = \text{Exp}\left(\mathbf{G}(t_i) \Delta t_i \right) 
% \end{align}
% We can then express this Jones matrix as a function of projected stress at $t_i$ by substituting $\mathbf{G}(t)$ from Eq.~\ref{eq:G_sig_tau}:
% \begin{align}
%     \mathbf{J}(t_i) = \text{Exp}\left(-i \frac{2\pi C}{\lambda}
% \begin{bmatrix}
% \sigma(t) & \tau(t) \\
% \tau(t) & -\sigma(t) 
% \end{bmatrix} \Delta t_i \right)  
% \label{eq:J_G}\;.
% \end{align}
% In App.~\ref{app:exp_j_A}, we show that Eq.~\ref{eq:J_G} can be simplified as,
% \begin{equation}
% \mathbf{J}(t_i) = \cos \left( -\frac{2\pi C}{\lambda} \sqrt{\sigma_{i}^2 + \tau_{i}^2} \right) \mathbf{I} 
% + I \frac{\sin \left( -\frac{2\pi C}{\lambda} \sqrt{\sigma_{i}^2 + \tau_{i}^2} \right)}{\sqrt{\sigma_{i}^2 + \tau_{i}^2}} G_{i}
% \end{equation}
% where we denote $\sigma(t_i)$ and $\tau(t_i)$ as $\sigma_i$ and $t_i$ respectively.
% We define the parameters $\delta_i$ and $\theta_i$ that are termed in the photoelastic literature as isochromatic and isoclinic parameters \cite{ramesh2021developments}.
% \begin{align}
% \delta_i = -\frac{4\pi C}{\lambda} \sqrt{\sigma_i^2 + \tau_i^2} \quad \quad 
% \theta_i = \frac{1}{2} \tan^{-1} \left( \frac{\sigma_{i}}{\tau_{i}} \right)
% \label{eq:delta_theta}
% \end{align}
We can express the Jones matrix in terms of these parameters as,
\begin{equation}
\mathbf{J}\left(t_i\right) = \cos \left(\nicefrac{\delta_i}{2}\right)
\begin{bmatrix}
1 & 0 \\
0 & 1
\end{bmatrix}
+ i \sin \left(\nicefrac{\delta_i}{2}\right)
\begin{bmatrix}
\cos 2\theta_i & \sin 2\theta_i \\
\sin 2\theta_i & -\cos 2\theta_i
\end{bmatrix}
\label{eq:J_retarder} \; ,
\end{equation} 
Aggregating along the entire ray, we can express the equivalent Jones vector $\mathbf{J}_\mathrm{eq}$ as the series of complex matrix multiplications,
\begin{equation}
\mathbf{J}_\mathrm{eq} = \prod_{i=1}^{N} \mathbf{J}(t_i) \;.
\label{eq:integrated_photoelasticity_Jones}
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/f1_formulation_and_approach/poincare_v1.pdf}
    \caption{\textbf{Modeling integrated photoelasticity.} By ray marching, we sample points along the queried ray (a). We model each segment between the sampled points,$t_{i}$ and $t_{i+1}$ as a retarder with retardance $\delta_i$ and slow-axis orientation $\theta_i$ (b). From Poincaré equivalence theorem, stack of any number of retarders is equivalent to a single retarder with parameters $(\delta_{\textit{eq}},\theta_{\textit{eq}})$ followed by a rotator with rotation $\gamma_{\mathrm{eq}}$ (c).}
    \label{fig:equivalence_theorem}
\end{figure}
\paragraph{Employing equivalence theorem} The net Jones matrix can be understood as a combination of $N$ retarders along the ray each with a different retardance $\delta_i$ and orientation $\theta_i$. Poincare's equivalence theorem states that the polarization properties of a combination of retarders are equivalent to that of a retarder followed by a rotator. Thus, the aggregate Jones matrix $\mathbf{J}_{\mathrm{eq}}$ can be represented by the product of Jones matrix of retarder with retardance $\delta_\mathrm{eq}$ and orientation $\theta_\mathrm{eq}$ and a rotator with $\gamma_\mathrm{eq}$.  The angles $\delta_\text{eq}$, $\theta_\text{eq}$ , and $\gamma_\text{eq}$  are denoted as the characteristic parameters \cite{aben1979integrated}. In App.~\ref{app:equivalence}, we derive the equivalence theorem for Eq.~\ref{eq:integrated_photoelasticity_Jones} and show that equivalent Jones matrix $\mathbf{J}_\text{eq}$ can be expressed based on the characteristic parameters as     
\begin{align}
\mathbf{J}_\text{eq} &= 
\cos{\left(\nicefrac{\delta_\text{eq}}{2}\right)}
\begin{bmatrix}
\cos 2\gamma_\text{eq} & \sin 2\gamma_\text{eq}\\
\sin 2\gamma_\text{eq} & -\cos 2\gamma_\text{eq} 
\end{bmatrix}  \nonumber \\
&+ i \sin{\left(\nicefrac{\delta_\text{eq}}{2}\right)} 
\begin{bmatrix}
\cos 2\theta'_\text{eq} & \sin 2\theta'_\text{eq}\\
\sin 2\theta'_\text{eq} & -\cos 2\theta'_\text{eq} 
\end{bmatrix} 
\label{eq:J_eq} \;,
\end{align}
where $\theta'_\text{eq} = \theta_\text{eq} - \gamma_\text{eq}$.
This matrix $\mathbf{J}_\text{eq}$  is composed of four unique elements denoted as $a$, $b$, $c$, and $d$ that depend on the characteristic parameters as :
\begin{align}
    a &= \cos{\left(\nicefrac{\delta_\text{eq}}{2}\right)}\cos 2\gamma_\text{eq}   & 
    b &= \cos{\left(\nicefrac{\delta_\text{eq}}{2}\right)}\sin 2\gamma_\text{eq}  \notag \\
    c &= \sin{\left(\nicefrac{\delta_\text{eq}}{2}\right)}\cos 2\theta'_\text{eq}  &
    d &= \sin{\left(\nicefrac{\delta_\text{eq}}{2}\right)}\sin 2\theta'_\text{eq} 
    \label{eq:abcd}
\end{align}
To simplify the derivations, we denote the $\mathbf{J}_\text{eq}$ based on its unique elements as 
\begin{align}
\mathbf{J}_\text{eq} &= 
\begin{bmatrix}
a & b \\
b & -b 
\end{bmatrix}  
+ i  
\begin{bmatrix}
c & d \\
d & -c 
\end{bmatrix} 
\label{eq:J_abcd} \;.
\end{align}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/f1_formulation_and_approach/general_vs_linear_model.pdf}
    \caption{\textbf{General vs linear 3D photoelasticity model.} The proposed general 3D photoelasticity formulation involves converting projected stress tensors at each point on the ray to Jones matrices (\textit{first phase wrap}) that are then integrated using matrix multiplications (\textit{then aggregate}). We also derive a first-order approximation of this model that involves first summing the projected stress tensors (\textit{first aggregate}) and then converting aggregated stress tensor to Jones matrix (\textit{then phase wrap})\ad{Need to link equations here.}. \textcolor{red}{we keep talking abt linear model and non-linear model but dont explicitly say why or how the non-linear model is better etc...need to make sure we emphasize that}}
    \label{fig:general_vs_linear}
\end{figure}

\paragraph{Linear approximation} In App.~\ref{app:first_order_approx}, we show that under first-order approximations, our formulation simplifies to a linear combination of projected stress followed by phase wrapping. Prior works leverage this approximation to formulate photoelastic tomography as linear tensor tomography \cite{szotten2011limited,sharafutdinov2012integral}. Consider the projected stress components $\sigma_{\text{lin}}$ and $\tau_{\text{lin}}$ defined as
\begin{equation}
\sigma_{\text{lin}} = \sum_{i=1}^{N} \sigma_i \Delta t_i
\quad \quad
\tau_{\text{lin}} = \sum_{i=1}^{N} \tau_i \Delta t_i
\label{eq:sig_tau_lin}
\end{equation}
In App~\ref{app:first_order_approx}, we also show that the aggregated Jones matrix under first-order approximation $\mathbf{J}_{\text{lin}}$ can be written as 
\begin{equation}
\mathbf{J}_{\text{lin}} = \cos \delta_{\text{lin}}/2 \mathbf{I} + j \sin \delta_{\text{lin}}/2
\begin{bmatrix}
\cos 2\theta_{\text{lin}} & \sin 2\theta_{\text{lin}} \\
\sin 2\theta_{\text{lin}} & -\cos 2\theta_{\text{lin}}
\end{bmatrix}
\label{eq:J_approx} \;,
\end{equation}
where
\begin{align}
\delta_{\text{lin}} = -\frac{4\pi C}{\lambda} \sqrt{\sigma_{\text{lin}}^2 + \tau_{\text{lin}}^2} \quad \quad 
\theta_{\text{lin}} = \frac{1}{2} \tan^{-1} \left( \frac{\sigma_{\text{lin}}}{\tau_{\text{lin}}} \right)
\end{align}
\label{eq:delta_theta}
\paragraph{Our general formulation vs linear approximation} In the most general case, the projected stress tensor at each point is encoded as Jones matrices (Eq.~\ref{eq:J_eq}) where there is phase wrapping of stress values due to sinusoidal expressions. Then all Jones matrices are aggregated using Jones matrix multiplication. The linear approximation employed by prior works (\cite{szotten2011limited,sharafutdinov2012integral}), first aggregates the projected stress values using Eq.~\ref{eq:sig_tau_lin} and then does phase wrapping (Eq.~\ref{eq:J_approx}). 

Due to \textit{first aggregate then phase wrap}, prior works rely on first phase wrapping the projected J value and then perform linear tensor tomography. Our \textit{first phase wrap and then aggregate} enables first tomography and then phase wrapping. When solving the inverse problem of reconstructing stress from Jones matrix, we can thus perform phase unwrapping in stress space rather than in projected Jones space. Thus we can directly apply smoothness prior in stress space and obtain better reconstruction than \textit{first aggregate then phase wrap} approach \ad{Refine the claim and link result}. 

Moreover, the aggregated Jones matrix in the general case (Eq.~\ref{eq:J_eq}) is parametrized by three characteristic parameters $\delta_{net}$, $\theta_{net}$ and $\gamma_{net}$. Aggregated Jones matrix in linear case (Eq.~\ref{eq:J_approx}) is modeled as an equivalent retarder with parameters $\delta_{lin}$ and $\theta_{net}$ and no rotator. Thus the linear approximation is not sufficient to model the rotation of polarization due to integrated photoelasticity.


\subsection{Multi-axis Polariscopy}
\label{sec:polariscope}
% \wh{this should probably be a separate section}
% Fixed \textcolor{red}{AV: sudden jump here. perhaps a few sentences pointing out from the previous eqna whre the tie into measurements is would make the transition smoother.}

In Sec.~\ref{sec:integrated_photoelasticity}, we showed that the equivalent Jones matrix (Eq.~\ref{eq:J_eq})   for each ray encodes a projection of the stress distribution. Here we describe how to  measure this Jones matrix through a polariscope-based capture setup comprising a linear polarizer and quarter waveplate before and after the target. We then describe how rotating the object and capturing polariscope measurement for each rotation enables photoelastic tomography.

\paragraph{Circular polariscope}
% Setup is closer to the prototype Multi-axis rotation polariscope geometry
We consider a circular polariscope-based setup (Fig.~\ref{fig:render_multiple_views}) to capture components of the Jones matrix in Eq.~\ref{eq:J_net}. Light emitted by an area light source passes through a linear polarizer (LP1) with the polarization axis oriented at an angle $\alpha_1$ with respect to the horizontal. The linearly polarized light then passes through a quarter wave plate (QWP1) with fast axis oriented at an angle $\beta_1$ with respect to the horizontal. The resulting circularly polarized light passes the specimen under stress. The light ray coming out of the specimen passes through another quarter wave plate (QWP2) with fast axis oriented at an angle $\beta_2$ and then reaches the polarization camera. The polarization camera comprises of a grid of linear polarizers at different orientations. Consider this light ray hits a sensor pixel which has a linear polarizer (LP2) oriented at an angle $\alpha_2$ with the horizontal.

\paragraph{Captured intensity}
Consider $\mathbf{E}(\alpha_1)$ as the Jones vector of light emitted from the LP1 and $\mathbf{Q}(\beta_1)$,$\mathbf{Q}(\beta_2)$ and $\mathbf{L}(\alpha_2)$ as the Jones matrices of QWP1, QWP2 and LP2 respectively. The effective Jones matrix as derived in Eq.~\ref{eq:J_net} depends on the characteristic parameters $\delta_{net}$, $\theta_{net}$ and $\gamma_{net}$.
The refraction into and outside the object also alters the polarization state based on the surface normals at those points. At the entry and exit points of the ray, $t_n$ and $t_f$, consider the Jones matrix depending on the surface normals $\mathbf{R}(t_n)$  and $\mathbf{R}(t_f)$.
Using Jones Calculus, the Jones vector of light reaching the sensor $\mathbf{E}_\text{cap}$ is given by the complex matrix multiplication:
\begin{align}
    \mathbf{E}_{\text{cap}} = \mathbf{L}(\alpha_1)\mathbf{Q}(\beta_1)\mathbf{R}(t_n)\mathbf{J}_{\text{eq}}\mathbf{R}(t_f)\mathbf{Q}(\beta_2)\mathbf{E}(\alpha_2)
    \label{eq:E_cap}
\end{align}
The captured intensity on the detector $I_d$ can be obtained from the Jones vector $\mathbf{E}$ by combining net intensity along orthogonal dimensions $\mathbf{u}$ and $\mathbf{v}$. 
\begin{align}
    I_\text{cap} = E_\mathbf{u}E_\mathbf{u}^* + E_\mathbf{v}E_\mathbf{v}^*
    \label{eq:I_cap}
\end{align}
By varying the polariscope element angles $\alpha_1$, $\beta_1$, $\beta_2$ and $\alpha_2$, we can obtain multiple intensity measurements that encode the characteristic parameters $\delta_{\text{net}}$, $\theta_{\text{net}}$ and $\gamma_{\text{net}}$.

\paragraph{Phase shifting technique}
To acquire the parameters of the Jones matrix $\mathbf{J}_\text{eq}$, we consider the phase shifting technique \cite{patterson1991towards} that is common in 2D photoelasticity and is extended to integrated photoelasticity \cite{tomlinson2002use}. Here the refraction effects at the boundaries of the object are neglected by either placing the object in a refractive index matched liquid \cite{abrego2019experimental} or assuming thin surfaces. LP1 is fixed at an orientation $\alpha = 90^\circ$. Measurements are obtained with varying rotations of QWP1, QWP2 and LP2. By leveraging snapshot polarization cameras we can acquire four rotations of LP2 simultaneously ($\alpha_2 = 0, \nicefrac{\pi}{4}, \nicefrac{\pi}{2}, \nicefrac{3\pi}{4}$). We consider two rotations of QWP1 ($\beta_1 = \nicefrac{\pi}{4}, \nicefrac{\pi}{2}$) and two rotations of QWP2 ($\beta_2 = 0, \nicefrac{\pi}{4}$). This results in 4 raw mosaiced measurements on the sensor that are demosaiced to obtain a total of 16 measurements which we denote as $I_1, I_2 \ldots I_{15} $. These 16 measurements depend on the 4 unique elements of the Jones matrix $\mathbf{J}_\text{eq}$ $a, b, c, d$ in a non-linear manner. From Eq. \ref{eq:J_abcd},\ref{eq:E_cap} and \ref{eq:I_cap}, we derive the expressions for the 16 measurements summarized in Table~\ref{table:intensity_abcd}. Please refer to App.~\ref{app:phase_shiftin_technique}, for details of this derivation and additional insights.  
\input{tables/captured_measurements_abcd}
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/f1_formulation_and_approach/captured_measurements.pdf}
    \caption{\textbf{Tomographic polariscope capture setup} By varying yaw-pitch rotations of the specimen and varying rotations of quarter waveplates and polarizers (a), we capture intensity measurements (b) that encode projections of the underlying stress tensor field.}
    \label{fig:render_multiple_views}
\end{figure}
\paragraph{Multi-rotation measurements}
The polariscope measurements described above (Table~\ref{table:intensity_abcd}) encode the equivalent Jones matrix $\mathbf{J}_\text{eq}$ (Eq~\ref{eq:J_abcd}) for each camera ray. This Jones matrix in turn depends on the projection of the stress tensors of the points along the ray (Eq~\ref{eq:projected_stress}). Every ray measures only a $2\times2$ projection of the $3\times3$ stress tensors on a plane perpendicular to that ray (Eq.~\ref{eq:projected_stress}). Therefore, to obtain the full $3\times3$ stress tensor at each point, we need to probe every point with multiple rays, each providing a different $2\times2$ projection of the $3\times3$ tensor. To obtain all possible $2\times2$ projections, the probing rays should be uniformly sampled from a unit hemisphere. 

To obtain multiple projections of the stress tensor field, we could either rotate the viewing camera rays by moving the camera and the screen around the object or we could rotate the object. In Fig.~\ref{fig:render_multiple_views}, we visualize the later case. Yaw rotation $\rho_1$ and pitch rotation $\rho_2$ of the object are equivalent to fixing the object and rotating the elevation and azimuth direction of the camera ray respectively. Thus by multiple yaw-pitch rotations of the object, we capture multiple projections of the stress tensor field enabling photoelastic tomography. 

\paragraph{Summarizing our capture setup}
Putting it all together, our capture scheme (Fig.~\ref{fig:render_multiple_views}) has two components: 1) yaw-pitch rotations of the object $\rho_1$, $\rho_2$  and 2) polariscope measurements involving rotations of QWP1 ($\beta_1$) and QWP2 ($\beta_2$) for each yaw-pitch rotation. Fig.~\ref{fig:render_multiple_views}(b) shows rendered images from our capture scheme for a disk under diametral compression. 

% This can be obtained either by rotating the object along its center or by moving the polariscope setup around the specimen.  In Fig.~\ref{fig:cir_pol}, we visualize the format  , but the formulation also holds true for the former case. 
% We consider moving the polariscope setup such that the camera is always pointed towards the center of the specimen and , along with QWP2, is moving along the surface of a sphere. The light screen, LP1 and QWP1 are also moving on the same sphere while being opposite the camera. Due to Helmholtz reciprocity, the camera only needs to move along one hemisphere while the light screen moves on the other hemisphere. The light rays probing the specimen are similar to that of a spherical light field. We parametrize the camera movement by azimuth and elevation rotation angles $\rho_\text{az}$ and $\rho_\text{el}$ respectively.

% yinput{tables/captured_16_measurements}

% The latter four equations can be combined as shown below to yield the isoclinic parameter, $\theta$

% \begin{equation}
% \theta - \gamma = \frac{1}{2} \arctan \left( \frac{I_5 - I_3}{I_4 - I_6} \right) 
% \end{equation}

% The obtained $\theta$ value can then be used to estimate the isochromatic parameters $\delta$,

% \begin{equation}
% \delta = \arctan \left( \frac{I_4 - I_6}{(I_1 - I_2) \cos 2(\theta- \gamma)} \right) 
% % = \arctan \left( \frac{I_5 - I_3}{(I_1 - I_2) \sin 2\theta} \right)
% \end{equation}


\begin{comment}
\begin{align}
\hat{\theta}-\hat{\gamma} &= 0.5 \cdot \tan^{-1}\left(\frac{I_3 - I_1}{2I_0 - I_3 - I_1}\right) \\
\hat{\delta} &= \tan^{-1}\left(\frac{I_3 - I_1}{(2I_2 - I_3 - I_1) \cdot \sin[2(\hat{\theta}-\hat{\gamma})]}\right) \\
\hat{\theta}+\hat{\gamma} &= 0.5 \cdot \tan^{-1}\left(\frac{I_3 + I_1 - 2\left(\frac{I_5}{\sin[2(\hat{\theta} + \hat{\gamma})]}\right) - \sin[2(\hat{\theta}-\hat{\gamma})]\cos(\hat{\delta})}{\cos[2(\hat{\theta}-\hat{\gamma})]}\right)^{-1}
\end{align}
, where $\sin[2(\hat{\theta} + \hat{\gamma})] = \frac{2I_4 - I_3 - I_1}{\sin(\hat{\delta})}$

From these parameters we can estimate the unique elements of Jones matrix:
\begin{align}
a &= cos(\hat{\delta})cos(2\hat{\gamma})\\
b &= sin(\hat{\delta})cos(2\hat{\gamma})\\
c &= sin(\hat{\delta})sin(2\hat{\theta})\\
d &= cos(\hat{\delta})sin(2\hat{\theta})\\
J_{\text{net}}  &= 
\begin{bmatrix}
a & d \\
d & -a 
\end{bmatrix}
+ j 
\begin{bmatrix}
b & c \\
c & -b
\end{bmatrix}
\end{align}
\end{comment}

==> sections/old/s5_recon_approach_v1.tex <==
\section{Neural Stress Tensor Tomography}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/figure_sketches/pipeline.png}
    \caption{Neural Stress Tomography Pipeline}
    \label{fig:pipeline}
\end{figure}
Here we describe our approach to reconstruct 3 dimensional stress tensor distribution from multi-view photoelastic measurements. We first introduce modeling stress tensor field $S(\mathbf{p})$ as neural implicit representation and how we can use the developed integrated photoelasticity model to render the projected Jones matrix $\mathbf{J}_{\text{net}}$ of the sample from these representations. We then show how we can estimate the captured aggregate Jones matrix from the captured intensity measurements $I_{d}$ along each ray.
\subsection{Neural stress fields}
 The stress field can vary dramatically throughout the object. For example, when an external load is applied on the object's boundary stress is often concentrated close to the boundary and then becomes sparse towards the bulk of the object (\ad{Cite Figure}). Representing this stress distribution requires adaptive sampling points in the object. For the stress tomography problem, as the stress is completely unknown at the start, this adaptive sampling cannot be fixed and known. We leverage the recent advancements in implicit neural representations to model complex visual distributions with high expressive power and computational efficiency.
 
 Stress at each point $\mathbf{p}$ within the object is modeled as a second-order symmetric tensor (Eq.~\ref{eq:stress_tensor}). We express this distribution with a coordinate-based MLP network $S$ with weights $\Theta$ that takes the position $\mathbf{p}$ as input and outputs the components of the Stress tensor matrix :
 \begin{align}
    S_{\Theta} : \mathbf{p} \rightarrow (\sigma_{xx}, \sigma_{yy}, \sigma_{zz}, \sigma_{xy}, \sigma_{yz}, \sigma_{zx})
 \end{align}
\subsection{Rendering aggregate Jones matrices from neural stress fields}
Our proposed Monte-Carlo formulation for integrated photoelasticity (Sec.~\ref{sec:integrated_photoelasticity}) is well-suited for rendering from continuous implicit stress distributions. \ad{Cite figure showing renderings}
\paragraph{Monte-Carlo Jones matrix multiplications}
For each ray $(\mathbf{o}, \mathbf{d})$ we sample $N$ points using stratified sampling between the object boundaries $(t_n, t_f)$. For every point $t$, we query the stress tensor $S_{\Theta}(t)$ and obtain the Jones matrix $\mathbf{J}(t)$ from Eq.~\ref{eq:J_retarder}.
From Eq.~\ref{eq:integrated_photoelasticity_Jones}, the projected Jones matrix can be obtained by complex matrix multiplications of Jones matrices along the ray
\begin{align}
    \mathbf{J}_\text{net} = \prod_{i=1}^{N} \mathbf{J}(t_i) \;.
\end{align}
\paragraph{Efficient rendering leveraging Poincare Equivalence Theorem}
Multiplying complex $2\times2$ Jones matrices along the ray can be computationally expensive. We show that these computations can be simplified by exploiting the structure of these Jones matrices. Using Poincare Equivalence Theorem, we show that this cascaded complex matrix multiplication can be broken down into an iterative accumulation of 4 scalar values along the ray.
The projected Jones matrix $\mathbf{J}_\text{net}$ (Eq.~\ref{eq:J_net}) has only 4 unique elements defined as
\begin{align}
   j_1^\text{net} &= \cos \delta \cos 2\gamma \\
   j_2^\text{net} &= \cos \delta \sin 2\gamma \\
   j_3^\text{net} &= \sin \delta \cos 2\theta \\
   j_4^\text{net} &= \sin \delta \sin 2\theta \;,
   \label{eq:unique_elements_j}
\end{align}
and the vector $\mathbf{j}_\text{net}$ as 
\begin{align}
    \mathbf{j}^\text{net} = [j_1^\text{net}, j_2^\text{net}, j_3^\text{net}, j_4^\text{net}]^T
    \label{eq:j_vec}
\end{align}
Similarly each intermediate Jones matrix $\mathbf{J}(t_i)$ from Eq.~\ref{eq:J_retarder}, can be written with three unique scalars $j^i_1, j^i_2,j^i_3$. In App.~\ref{app:equivalence}, we derive using Poincare equivalence thereom, that unique elements $\mathbf{j}\text{net}$ can be obtained by iteratively accumulating four scalar elements $ \mathbf{k}^i = [k^i_1, k^i_2, k^i_3, k^i_4]^T$, such that
\begin{align}
    \mathbf{k}^0 &= [1, 0, 0, 0]^T \\
    \mathbf{k}^i &=  M(\mathbf{j}^i)\mathbf{k}^{i-1}\\
    \mathbf{j}^{\text{net}} &=  \mathbf{k}^N \;,
\end{align}
where $M$ a matrix composed of elements from $\mathbf{j}^i$ as described in App.~\ref{app:equivalence}.

\subsection{Estimating projected Jones matrices from captured intensity measurements}
The above rendering scheme allows us to render the projected Jones matrix $\mathbf{J}_\text{net}$ from the unknown stress distribution. We aim to compare this to the captured projected Jones matrix $\mathbf{J}_\text{cap}$. As shown in Sec.~\ref{sec:integrated_photoelasticity} the projected Jones matrix along each ray depends on three characteristic parameters $\delta_\text{net}$, $\theta_\text{net}$ and $\gamma_\text{net}$. 
\paragraph{Estimated characteristic parameters}
These parameters are encoded in the captured intensity measurements. For the case of six-step phase shifting, we can analytically estimate the  parameters \cite{tomlinson2002use} as:
\begin{align}
\hat{\theta}-\hat{\gamma} &= \frac{1}{2} \tan^{-1}\left(\frac{I_3 - I_1}{2I_0 - I_3 - I_1}\right) \\
\hat{\delta} &= \tan^{-1}\left(\frac{I_3 - I_1}{(2I_2 - I_3 - I_1) \sin2(\hat{\theta}-\hat{\gamma})}\right) \\
\hat{\theta}+\hat{\gamma} &= \frac{1}{2}\tan^{-1}\left(\frac{\cos2(\hat{\theta}-\hat{\gamma})}{I_3 + I_1 - \frac{2 I_5}{\sin2(\hat{\theta} + \hat{\gamma})} - \sin2(\hat{\theta}-\hat{\gamma})\cos\hat{\delta}}\right)
\end{align}
, where $\sin2(\hat{\theta} + \hat{\gamma}) = \frac{2I_4 - I_3 - I_1}{\sin\hat{\delta}}$. 
\paragraph{Pi ambiguity}
Due to the $tan^{-1}$ operations, the estimated parameters are wrapped to the range of $[0, \pi]$ and exhibit a $\pi$ ambiguity with the ground truth characteristic parameters that are in the range $[0,2\pi]$
\begin{align}
    \hat{\delta} &= \delta \quad \text{or} \quad \delta + \pi/2 \quad \text{or} \quad \delta + 3\pi/2 \quad \text{or} \quad \delta + \pi \\
    \hat{\theta} &= \theta \quad \text{or} \quad \theta + \pi \\
    \hat{\gamma} &= \gamma \quad \text{or} \quad \gamma + \pi \\
\end{align}
\paragraph{Estimated projected Jones matrix}
From Eq.~\ref{eq:J_net}, we can estimate the projected Jones matrix along the ray $\hat{\mathbf{J}_\text{cap}}$ from the estimated characteristic parameters. Due to sine and cosine terms in the projected Jones matrix, the $\pi$ ambiguity in estimated characteristic parameters results in a sign ambiguity in the projected Jones matrix. In particular for the unique elements of the Jones matrix defined in Eq.~\ref{eq:unique_elements_j}, we have the following ambiguity
\begin{align}
    [j^\text{cap}_1, j^\text{cap}_2] &= [\hat{j}^\text{cap}_1, \hat{j}^\text{cap}_2] \quad \text{or} \quad [-\hat{j}^\text{cap}_1, -\hat{j}^\text{cap}_2] \\
    [j^\text{cap}_3, j^\text{cap}_4] &= [\hat{j}^\text{cap}_3, \hat{j}^\text{cap}_4] \quad \text{or} \quad [-\hat{j}^\text{cap}_3, -\hat{j}^\text{cap}_4] 
\end{align}
\ad{Need to add the case with all 12 snapshot polarization camera measurements and handling refraction effects.}
\subsection{Reconstructing neural stress field from projected Jones matrices}
\paragraph{Adaptive sampling}
Neural implicit representations enable us to sample during the reconstruction process only the regions that contain stress. Similar to InstantNGP \cite{muller2022instant}, we learn a binary coarse occupancy grid $\mathbf{B}$ jointly with the implicit stress field. This occupancy grid is trained to have high values when the tensor norm at that point exceeds a threshold $\epsilon$
\begin{align}
    \mathbf{B}(\mathbf{p}) = \mathbf{S}(\mathbf{p}) > \epsilon
\end{align}
The neural stress field is then queried more frequently at points with high occupancy thereby reducing the sampling of empty stress regions.
\paragraph{Loss functions and regularization}
We define the loss between the rendered projected Jones matrix $\mathbf{J}_{\text{net}}$ and the captured projected Jones matrix $\mathbf{J}_{\text{cap}}$ as the L1 loss between their unique elements $\mathbf{j}^{\text{cap}}$ and $\mathbf{j}^{\text{net}}$.
As the jones matrix have sign ambiguity we define a loss on the absolute values of these vectors, $\mathcal{L}_\text{jones}$
\begin{align}
    \mathcal{L}_\text{jones } = \sum_{\text{all rays}} \||\mathbf{j}^{\text{cap}}| - |\mathbf{j}^{\text{net}}| \|_1
\end{align}

==> sections/old/s6_results_v1.tex <==
\section{Simulation Results and Analysis}
In this section, we discuss simulation experiments on synthetic datasets and the implementation of the pipeline in more detail. With simulation, we qualitatively compare against ground truth reference data, and also quantitatively analyze the performance of our method under a few key factors. 

\subsection{Simulated 3D Photoelasticity Dataset}
First, to exclude areas outside each object and handle discontinuity, we fit a 3D object mask that maps a 3D point (x,y,z) to 0 or 1, indicating whether the 3D point is inside the object. For each object, we fit a SIREN network \cite{sitzmann2020implicit} on the surface point cloud as well as the normals, to output SDF values. We used a SIREN network with 3 hidden layers and 256 neurons, which has enough capacity to fit the SDF of the complex 3D shape of TSV objects. 

To obtain the occupancy mask, we then threshold the SDF outputs from the SIREN network such that negative SDF values result in 1 and positive SDFs (outside object) result in 0. For irregular shapes, this step is necessary to avoid out-of-object ray points from corrupting rendered images and could also help handle stress discontinuity at object surfaces. For box-like shapes, one can skip the fitting step and directly use a box shape to confine the effective region.

We perform efficient rendering using Instant-NGP \cite{muller2022instant} for coarse-to-fine 3D sampling. We then query the stress field at each ray point and follow formulations in Section 4 to render the intensity images. Note that occupancy is used in both (1) the rendering stage to mask stress field values directly and (2) Instant-NGP to exclude low occupancy regions and accelerate sampling. To be specific, instead of having Instant-NGP jointly learn the binary occupancy grid, we directly initialize the grid from SIREN and fix it during optimization. 

To query the stress tensor at any arbitrary point, we interpolate tensor values from nearby sample points. The sample stress field data usually comes in two formats. \textbf{Regular grid} can be used where each grid point has an associated stress tensor. A new point can directly sample from the vertices of the grid it falls in. 

Another case is FEM outputs. FEM simulation often outputs \textbf{non-uniform} sampled data such as meshes or Cartesian grids. To reduce memory throughput, the points and surfaces are sampled adaptively, whereas regions with high-frequency stress changes are sampled more densely. To handle interpolation here, we use K-Nearest Neighbors (KNN) sampling. For each ray point, we search for its $k$ nearest neighbors ($k\geq 3$) among the original FEM sample points and interpolate the stress tensors. KNN algorithms can be run very efficiently, thanks to the use of tree structures and algorithmic accelerations such as parallelism. Once the neighbors are found, the new sample point takes on the weighted average of the stress values of the K neighboring points, where the weights are inversely proportional to the squared distance to the sample point. 

% During the interpolation, it is important to guarantee that the stress tensor elements sum to 0. Hence we consistently use linear interpolation. 
To reconstruct the underlying neural stress field, we take the rendered images and optimize a neural field that is an implicit representation of the stress values. We minimize error between the observations and the measurement rendered from the neural stress field $S$, with respect to the weights of the network $\Theta$. 

% \paragraph{Toy Datasets}
% \textcolor{green}{Akshat TODO}
% Gaussians? disks?

\paragraph{FEM Scenes}
We evaluate 3D stress field reconstruction for complex shapes using the 3D-TSV dataset \cite{wang20223d}. 3D-TSV includes several common objects and mechanical parts. Each example object is represented by adaptively sampled hexagonal mesh or Cartesian grids. We take the vertices and the 6D stress tensors associated with them as our ground truth. We first normalize the coordinates and stress values to fall between 0 to 1. We perform a series of rendering and reconstruction experiments on femur and bearing. The phase wrapping coefficients are chosen to be 0.5 for femur and 0.25 for bearing to generate reasonably dense fringes.  \textcolor{green}{tz: might add cantilever as the 3rd object. Coeff = 0.1. Render step size is 5e-3 for canti and 1e-2 for the rest. }. We show qualitative comparisons on all objects. We also perform a detailed analysis of the femur object. Each object is rendered with 32 azimuth angles and 32 elevation angles, with a full 180-degree view range along each axis. 

For this dataset, each sample takes about 2 hours to render on an A100 GPU. 

In the following paragraphs, we analyze the performance of our method using both toy dataset and TSV samples. We evaluating the performance qualitatively,and we quantitatively analyze the effect of several important factors: the amount of phase wrapping, scanning angle, and reconstruction method (linear vs. non-linear).

\textcolor{green}{AD: discuss end-to-end/e2etomowrap or point to which recon method is used? (not sure how it's being referred to in earlier sections). Make sure they are categorized correctly into qualitative vs quantitative}



% AY: Putting here for now
% \begin{comment}
% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{figures/f3_sim_results/sim_showcase.pdf}
%     \caption{\textbf{Stress visualization of a synthetic bracket} We employed multiple visualization (\textcolor{green}{Tianyi: do we need this Figure still?}) }
%     \label{fig:sim_showcase}
% \end{figure*}

% \end{comment}
% 3D TSV pipeline
\subsection{Qualitative Comparison}

For qualitative comparison, we use the full 32x32 renderings with the full 180-degree range on each axis. The reconstructions are performed on all the 32x32 captures. In Fig. \ref{fig:sim_showcase} we qualitatively examine the stress field reconstruction against the ground truth. Fig. \ref{fig:sim_showcase} compares the simulation results. From (b), we can see that the optimization successfully matched the renderings from reconstructed stress fields and the images simulated directly from ground truth data. In (c), we visualize the reconstructed stress by the different tensor components and the principle stress decomposition. We can see that our reconstruction closely approximates the ground truth. The principle stress analysis shows the characteristics of the stress can be fully preserved with our method -- where we see the clear contact points of the compression and tension on the surfaces of the femur. In the two holes of the bearing, we can also see a sudden increase fo the force in both ground truth and our reconstruction. 

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/f3_sim_results/sim_analysis_coneangle.pdf}
    \caption{\textbf{The effect of varying rotation angles. } For each object, from left to right, we show the reconstructed stress field as we vary the range of angles we scan. We compare the reconstructions with each scanning configuration with the ground truth stress values and slices, as well as report the MSE for the stress field (in the region of occupied by the target). Here we only show the $\sigma_{xx}$}
    \label{fig:sim_analysis_rotation}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/f3_sim_results/sim_analysis_coeff_effect.pdf}
    \caption{\textbf{The effect of increasing phase wrapping.} More fringes can be observed in the rendered image as the warping coefficient increases. The reconstruction also gives more error once the fringes become dense enough, in this case when the warping coefficient reaches 0.5. The residuals of the reconstructed images are also much higher than the lower warping coefficients. }
    \label{fig:sim_analysis_coeff}
\end{figure*}

\subsection{Effect of rotation angles}
In tomography, the rotation angle or the scanning angle is important. Here we start with the hemisphere (180x180), and gradually reduce to a cone where the center aligns with the object. We reduce the angle of the cone (scanning range in each direction) from 180 down to 90 degrees on each direction (2X subsampling), and 45 degrees (4X subsampling). The effects are shown in Fig. \ref{fig:sim_analysis_rotation} below.  As the angle reduces, the quality of reconstruction reduces significantly. With 90 degrees, reasonable reconstruction can be obtained for most of the object. However, artifacts start to occur. When subsampling is 4X, the quality degrades significantly and distortions can be seen in the reconstructed stress field. Notice that the distortions on bearings are much more severe due to the bearing having more complexities in the stress field. For the femur, which has a smoother stress field, while distortions can be visually seen in slices but it doesn't contribute too much to the MSE fluctuations. For bearing the effect can be seen in both. 


The results match the observations in conventional tomography as well -- where the missing cone problem could significantly degrade the performance as unobserved angles increase. 


\subsection{Effect of phase wrapping}
We characterize the effect of phase wrapping using the bearing sample from the 3D-TSV dataset. We vary the phase wrapping coefficient for femur in the rendering stage from 0.1, 0.25 up to 0.5. To mimic real image effects, we also add a small, typical amount of iid Gaussian noise with 0 mean and variance of 0.01. An example rendered view is shown for each coefficient in Fig. \ref{fig:sim_analysis_coeff}. 

In addition to qualitatively comparing the reconstruction results, we also quantify the mean squared error (MSe) of the reconstructed stress field. We uniformly sample $N=101^3$ within the bounding box of the object, with the number of sampled values in each dimension to be N. We compute the MSE between the ground truth stress values sampled at these points vs. the reconstructed stress values queried at the same points. For the TSV dataset, the ground truth field can be represented by a KNN interpolator on the original sample points. The reconstructed stress field is in the form of a coordinate-based network. 



\section{Experiments and Results}

\begin{comment}
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figures/f3_sim_results/sim_scenes.pdf}
    \caption{\textbf{Simulated 3D photoelasticity dataset using 3D TSV stress data}}
\end{figure*}
\end{comment}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/hardware/acquisition_setup.pdf}
    \caption{\textbf{Proposed multi-axis polariscope setup.}  }
    \label{fig:acquisition_setup}
\end{figure}
\begin{figure}
    \centering
    \includegraphics{figures/f3_real_results/real_scenes.pdf}
    \caption{\textbf{Proposed 3D Photoelasticity experimental dataset}}
    \label{fig:real_scenes}
\end{figure}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/f3_real_results/real_qualitative_stacked_disk.pdf}
    \caption{\textbf{Qualitative comparison of reconstructions for experimental stacked compressed disks}}
    \label{fig:sim_qualitative_disk}
\end{figure*}
\begin{figure}
    \centering
    \includegraphics{figures/f3_real_results/app_visualization.pdf}
    \caption{\textbf{Application: Visualization of stress as photoelastic fringes along novel views}}
    \label{fig:app_visualizatino}
\end{figure}
\begin{figure*}
    \centering
    \includegraphics{figures/f3_real_results/appp_virtual_slicing.pdf}
    \caption{\textbf{Application: NeST can computationally decompose individual components of the specimen }}
    \label{fig:virtual_slicing}
\end{figure*}
\begin{comment}
  
\begin{figure}
    \centering
    \includegraphics{figures/f3_real_results/app_inspection.pdf}
    \caption{\textbf{Application: NeST 3D localize inhomogeneities based on the discontinuity in stress fields.}}
    \label{fig:enter-label}
\end{figure}
\end{comment}
% \begin{comment}
% \end{comment}
\begin{comment}
\begin{figure*}
    \centering
    \includegraphics{figures/f3_sim_results/sim_qualitative_results}
    \caption{\textbf{Stress reconstructed from images rendered using 3D-TSV dataset} We consider scenes in 3D TSV comprising of physics-based simulation of stress distribution in complex 3D objects (a). We render photoelastic images under varying polariscope elements and 3D object rotations (b). The estimated stress distribution from NeST match ground truth distribution as shown by slices of elements of the stress tensor and 3D visualization of the principal stress.}
    \label{fig:3d_tsv}
\end{figure*}
\end{comment}

% \subsection{Experimental Results and Comparisons}

\subsection{Acquisition setup}
% - Picture of the setup
% - Explain the capture procedure 

The acquisition setup is shown in \ref{fig:acquisition_setup}. As explained in Section~\ref{sec:polariscope}, the sample is imaged along two rotational axes: azimuth ($\rho_2$) and elevation ($\rho_1$). To minimize the footprint of the physical capture setup, instead of rotating the camera about the azimuth range, the object is rotated. This is identical to rotating the camera, however minimizes the horizontal space required for the system. Thus, the light panel and diffuser, linear polarizer and quarter wave plate, and the camera are all mounted coliniearly along a rod mounted to the elevation rotation stage such that all components move together.


Further, in order to capture all 
intensities depicted in Table~\ref{table:intensity_abcd}, each experiment contained a total of six total states. Each state had a unique configuration of light-side LP angle ($\alpha_1$), whether the QWP was on or not,  camera-side LP angle ($\beta_1$), and whether the 432nm bandpass filter was included. These states are shown in Table~\ref{table:acquisition_intensity_states}. 

\input{tables/acquisition_setup_intensites}

Based on the sample and current state, acquisition parameters were adjusted accordingly. For instance, when the bandpass filter was added, this necessitated an increase in exposure time to compoensate for the decreased total intensity. And if an external force was applied during capture, due to the force applicator occluding the object at specific angles, the total azimuth and/or elevation range would change.

\subsection{Test subjects}
% - Process of creating test subjects 
% -List of test subjects

The custom test subjects were made from a two-part epoxy resin and molded in various shapes using silicon molds. For simple shapes, off-the-shelf molds were utilized. For more complex shapes, including samples with letters or with strict dimensions, liquid silicon molds were cast around 3D printed parts, and the samples were then created in the same way as before. For test subjects which demonstrated residual stresses, these were simply chosen if they exhibited considerable stresses with fringing.

\paragraph{Samples with Residual Stresses}

Two types of samples with residual stresses were used: household transparent plastics and resin. The household objects were simply objects that are commonly found around the house, such as tape measures, transparent boxes, flat plastic dividers, etc. Due to the injection molded process used to manufacture these parts, residual stresses are common and the samples with the most birefringence were selected. The second type were resin samples. These were cast resin samples that had a compressive force applied for in excess of 24 hrs. Due to the nature of the resin we used, the samples would set and exhibit residual stresses even after the force was removed. These samples simplified the mounting setup and allowed for extended azimuth and elevation ranges.

\paragraph{Samples with Applied Stresses}

To apply an adequate force, custom 3D printed mounts were made which applied a compressive force on the samples. The mount was modeled such that it allows varying angle of applied stress on the XY-plane. Furthermore, the mount was created such that two samples could be mounted sequently along Z, as shown in Figure~\ref{fig:acquisition_setup}. Each force applicator could be removed indepently of the other to facilitate the capture of individual samples for validation (as in the front sample was captured, both samples were then captured together, and then the back sample was captured). To restrict the force applied to the sample to compression, a ball-and-socket nut was mounted to each screw such that no torsion was applied as the screw was tightened. 

\subsection{Qualitative Results}

In practice, analysis of an objects stresses is restricted to surface properties or visual inspection. Both methods fail to yield quantifiable data about the internal stress of an object. Via NeST, we are able to recover the internal stress field and subsequently analyze and visualize the properties of the specimen. We analyze two examples to quantatively benchmark our results: 1) a disk with two compressive loads on each face and 2) a triangular prism with loads partially along z (i.e. a shear load in addition to a compressive load is applied). These examples were chosen because they contain three dimensional information, as in they vary along the length of the speciman. For 1), it's expected that at the two faces, where the load is applied, you would see stresses similar to a single compressed disks. This is evident with the first and last slices in Figure~\ref{fig:real_qualitative_disk}.c. The second and third are then a combination of both stress profiles. A similar idea is present in the results for the triangular prism.

\subsection{NeST Applications}

\paragraph{Virtual Slicing}

Virtual slicing of 3D volumes is a common tool for analyzing stress fields and serves as an intuitive measure of the internal stresses within an object. An example of virtual slicing using NeST is shown in Figure~\ref{fig:appp_virtual_slicing}. With two objects stacked in line with one another, the photoelastic fringes are superimposed on one another and interfere. NeST is able to successfully decompose the fringes of each speciman, and their individual components can be extracted. This is shown with a simple scenario with compressed square and hexagonal prisms. A more complex example was tested where individual letter cutouts were extracted from specimens, which is challenging given the non-uniformity of the profiles around the sharp edges of the letters.

\paragraph{Novel Stress Visualization}

Virtual slicing can be thought of a novel view of the stress profile. This is because the slices are inherently new; only external data capture was used, and so any internal information is reconstructed from this data. In addition to slicing the objects at different points, you can virtually view the stress profile at various points and interpolate between the data captures. This is reminscent of NeRF novel view synthesis, and can be helpful in constructing a full 3D representation of the stress field. This is visualized in Figure~\ref{fig:app_visualization}, where novel views of complex geometires, such as a tape measure, are rendered from the photoelastic fringes.

\begin{comment}
    
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth,page=2]{figures/f4_analysis/sim_voxel_vs_inr.pdf}
    \caption{\textbf{Voxel grids vs implicit neural representations (INRs) to represent 3D scenes} We considered voxel grids and implicit neural representations as trainable data structures to model the 3D stress tensor field. We first fit a voxel grid and INR respectively to the ground truth stress field and render the corresponding Jones views. We then perform reconstruction, where the benefis of unconstrained sampling resolution with INRs become clear as the high frequencies of the images can't be reconstructed. This comparison is demonstrated on a simulated cylindrical object with axial loading.}
    \label{fig:sim-voxel-vs-inr}
\end{figure*}
\end{comment}

% Older analysis
\begin{comment}
\subsection{Tomography}
    \paragraph{Effect of Regularization}
\begin{figure}
    \centering
\includegraphics[width=\linewidth]{figures/f4_analysis/fig_reg_weight.pdf}
    \caption{\textbf{Effect of regularization weightages }}
    \label{fig:reg_weight}
\end{figure}
    \paragraph{Effect of Phase wrapping}
\begin{figure*}
    \centering
\includegraphics[width=\textwidth]{figures/f4_analysis/analysis_phase_wrapping.pdf}
    \caption{\textbf{Effect of increasing wrapping }}
    \label{fig:wrapping}
\end{figure*}
    \paragraph{Effect of number of rotation angles}
\begin{figure*}
    \centering
\includegraphics[width=\textwidth]{figures/f4_analysis/fig_angle_effects.pdf}
    \caption{\textbf{Effect of angles }}
    \label{fig:angles}
\end{figure*}
\end{comment}


% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}{.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/voxel_vs_inr_analysis/inr_from_gt_1_compressed_disks_2_coeff_05_reg_001.png}
%         \caption{}
%         \label{fig:inr_gt_fit}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/voxel_vs_inr_analysis/voxel_from_gt_1_compressed_disks_2_coeff_05_reg_001.png}
%         \caption{}
%         \label{fig:voxel_gt_fit}
%     \end{subfigure}
%     \caption{Comparison of the fitted stress of an axially compressed disk between  \subref{fig:inr_gt_fit}) an MLP and \subref{fig:voxel_gt_fit}) a voxel grid. }
% \end{figure}

% \begin{figure}
%     \centering
% \includegraphics[width=\textwidth]{placeholder.png}
%     \caption{Renderings and reconstructions on cantilever with varying wrapping coefficients (C). For each coefficient, the first Jones components of the initial view are shown. As more wrapping takes place in rendering, optimization becomes more difficult }
%     \label{fig:enter-label}
% \end{figure}



==> tables/acquisition_setup_intensites.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}lcccr@{}} % Added a new column for rho
\toprule
 State & \multicolumn{1}{c}{\textbf{$\alpha_1$ }} & \textbf{$QWP$ } & \textbf{$\beta_2$ } & Filter \\
\midrule

$1$ & $0$ & $Yes$ & $\pi/4$ \& $\pi/2$ & Yes \\
$2$ & $0$ & $No$ & $\pi/4$ \& $\pi/2$ & Yes \\
$3$ & $0$ & $No$ & $\pi/4$ & No \\
$4$ & $\pi/4$ & $No$ & $\pi/4$ & No \\
$5$ & $\pi/2$ & $No$ & $\pi/4$ & No \\
$6$ & $3\pi/4$ & $No$ & $\pi/4$ & No \\

\bottomrule
\end{tabular}
\caption{\textbf{Physical acquisition setup states.} Six total states were used when performing a capture. Our method utilizes States $1$ and $2$, where the previous methods use all 6.}
\label{table:acquisition_intensity_states}
\end{table}

==> tables/captured_16_measurements_v1.tex <==
\begin{comment}
\begin{table}[h]
\centering
\begin{tabular}{@{}clcc@{}} % Adjusts column spacing
\toprule
\textbf{Measurement} & \multicolumn{1}{c}{\textbf{$\eta$ values}} & \textbf{$\beta$ values} & \textbf{Intensity Expression} \\
\midrule
$I_1$ & 0 & 0 & $2\cos(\delta - 2\gamma + 2\theta) - 2\cos(\delta + 2\gamma - 2\theta) + 5$ \\
$I_2$ & 0 & $\pi/4$ & $5 - 4\cos(\delta)$ \\
$I_3$ & 0 & $\pi/2$ & $2\cos(\delta - 2\gamma + 2\theta) - 2\cos(\delta + 2\gamma - 2\theta) + 5$ \\
$I_4$ & 0 & $3\pi/4$ & $4\cos(\delta) + 5$ \\
$I_5$ & $\pi/4$ & 0 & $4\cos(\delta) + 5$ \\
$I_6$ & $\pi/4$ & $\pi/4$ & $2\sin(\delta - 2\gamma + 2\theta) + 2\sin(\delta + 2\gamma - 2\theta) + 5$ \\
$I_7$ & $\pi/4$ & $\pi/2$ & $5 - 4\cos(\delta)$ \\
$I_8$ & $\pi/4$ & $3\pi/4$ & $2\sin(\delta - 2\gamma + 2\theta) + 2\sin(\delta + 2\gamma - 2\theta) + 5$ \\
$I_9$ & $\pi/2$ & 0 & $-2\cos(\delta - 2\gamma + 2\theta) + 2\cos(\delta + 2\gamma - 2\theta) + 5$ \\
$I_{10}$ & $\pi/2$ & $\pi/4$ & $4\cos(\delta) + 5$ \\
$I_{11}$ & $\pi/2$ & $\pi/2$ & $-2\cos(\delta - 2\gamma + 2\theta) + 2\cos(\delta + 2\gamma - 2\theta) + 5$ \\
$I_{12}$ & $\pi/2$ & $3\pi/4$ & $5 - 4\cos(\delta)$ \\
$I_{13}$ & $3\pi/4$ & 0 & $5 - 4\cos(\delta)$ \\
$I_{14}$ & $3\pi/4$ & $\pi/4$ & $-2\sin(\delta - 2\gamma + 2\theta) - 2\sin(\delta + 2\gamma - 2\theta) + 5$ \\
$I_{15}$ & $3\pi/4$ & $\pi/2$ & $4\cos(\delta) + 5$ \\
$I_{16}$ & $3\pi/4$ & $3\pi/4$ & $-2\sin(\delta - 2\gamma + 2\theta) - 2\sin(\delta + 2\gamma - 2\theta) + 5$ \\
\bottomrule
\end{tabular}
\caption{Intensity expressions for different $\eta$ and $\beta$ values.}
\label{table:intensity_expressions}
\end{table}
\begin{table}[h]
\centering
\begin{tabular}{@{}clcc@{}} % Adjusts column spacing
\toprule
\textbf{Measurement} & \multicolumn{1}{c}{\textbf{$\eta$ values}} & \textbf{$\beta$ values} & \textbf{Intensity Expression} \\
\midrule
$I_1$ & 0 & 0 & $-2\cos(\delta - 2\gamma + 2\theta) + 2\cos(\delta + 2\gamma - 2\theta) + 5$ \\
$I_2$ & 0 & $\pi/4$ & $4\cos(\delta) + 5$ \\
$I_3$ & 0 & $\pi/2$ & $-2\cos(\delta - 2\gamma + 2\theta) + 2\cos(\delta + 2\gamma - 2\theta) + 5$ \\
$I_4$ & 0 & $3\pi/4$ & $5 - 4\cos(\delta)$ \\
$I_5$ & $\pi/4$ & 0 & $5 - 4\cos(\delta)$ \\
$I_6$ & $\pi/4$ & $\pi/4$ & $-2\sin(\delta - 2\gamma + 2\theta) - 2\sin(\delta + 2\gamma - 2\theta) + 5$ \\
$I_7$ & $\pi/4$ & $\pi/2$ & $4\cos(\delta) + 5$ \\
$I_8$ & $\pi/4$ & $3\pi/4$ & $-2\sin(\delta - 2\gamma + 2\theta) - 2\sin(\delta + 2\gamma - 2\theta) + 5$ \\
$I_9$ & $\pi/2$ & 0 & $2\cos(\delta - 2\gamma + 2\theta) - 2\cos(\delta + 2\gamma - 2\theta) + 5$ \\
$I_{10}$ & $\pi/2$ & $\pi/4$ & $5 - 4\cos(\delta)$ \\
$I_{11}$ & $\pi/2$ & $\pi/2$ & $2\cos(\delta - 2\gamma + 2\theta) - 2\cos(\delta + 2\gamma - 2\theta) + 5$ \\
$I_{12}$ & $\pi/2$ & $3\pi/4$ & $4\cos(\delta) + 5$ \\
$I_{13}$ & $3\pi/4$ & 0 & $4\cos(\delta) + 5$ \\
$I_{14}$ & $3\pi/4$ & $\pi/4$ & $2\sin(\delta - 2\gamma + 2\theta) + 2\sin(\delta + 2\gamma - 2\theta) + 5$ \\
$I_{15}$ & $3\pi/4$ & $\pi/2$ & $5 - 4\cos(\delta)$ \\
$I_{16}$ & $3\pi/4$ & $3\pi/4$ & $2\sin(\delta - 2\gamma + 2\theta) + 2\sin(\delta + 2\gamma - 2\theta) + 5$ \\
\bottomrule
\end{tabular}
\caption{Intensity expressions for different $\eta$ and $\beta$ values.}
\label{table:intensity_expressions}
\end{table}
\end{comment}
\begin{table*}[h]
\centering
\begin{tabular}{@{}cccccc@{}} % Adjusts column spacing
\toprule
\textbf{Measurement} & \textbf{$\beta$} & \textbf{$\eta$} & \textbf{$\alpha$} & \textbf{$\rho$} & \textbf{Intensity Expression} \\
\midrule
$I_1$ & 0 & 0 & 0 & 0 & $-2\cos(\delta - 4\gamma + 2\theta) + 2\cos(\delta + 4\gamma - 2\theta) + 5$ \\
$I_1$ & 0 & 0 & 0 & 0 & $5+4\sin(\delta)\sin(2\theta-4\gamma)$ \\
$I_2$ & 0 & 0 & $\pi/2$ & $\pi/4$ & $9\sin^2(0.5\delta)\sin^2(2(\gamma - \theta)) + \sin^2(0.5\delta)\cos^2(2(\gamma - \theta)) + 9\sin^2(2\gamma)\cos^2(0.5\delta) + \cos^2(0.5\delta)\cos^2(2\gamma)$ \\
$I_2$ & 0 & 0 & $\pi/2$ & $\pi/4$ & $$ \\
$I_3$ & 0 & $\pi/4$ & 0 & 0 & $4\cos(\delta) + 5$ \\
$I_4$ & 0 & $\pi/4$ & $\pi/2$ & $\pi/4$ & $2\cos(\delta - 2\theta) - 2\cos(\delta + 2\theta) + 5$ \\
$I_5$ & $\pi/4$ & 0 & 0 & 0 & $5 - 4\cos(\delta)$ \\
$I_6$ & $\pi/4$ & 0 & $\pi/2$ & $\pi/4$ & $-2\cos(\delta - 2\theta) + 2\cos(\delta + 2\theta) + 5$ \\
$I_7$ & $\pi/4$ & $\pi/4$ & 0 & 0 & $-2\sin(\delta - 4\gamma + 2\theta) - 2\sin(\delta + 4\gamma - 2\theta) + 5$ \\
$I_8$ & $\pi/4$ & $\pi/4$ & $\pi/2$ & $\pi/4$ & $2\sin(4\gamma) - \sin(\delta - 4\gamma) + \sin(\delta + 4\gamma) + 2\sin(4\gamma - 4\theta) + \sin(\delta - 4\gamma + 4\theta) - \sin(\delta + 4\gamma - 4\theta) + 5$ \\
$I_9$ & $\pi/2$ & 0 & 0 & 0 & $2\cos(\delta - 4\gamma + 2\theta) - 2\cos(\delta + 4\gamma - 2\theta) + 5$ \\
$I_{10}$ & $\pi/2$ & 0 & $\pi/2$ & $\pi/4$ & $2\cos(4\gamma) + \cos(\delta - 4\gamma) + \cos(\delta + 4\gamma) + 2\cos(4\gamma - 4\theta) - \cos(\delta - 4\gamma + 4\theta) - \cos(\delta + 4\gamma - 4\theta) + 5$ \\
$I_{11}$ & $\pi/2$ & $\pi/4$ & 0 & 0 & $5 - 4\cos(\delta)$ \\
$I_{12}$ & $\pi/2$ & $\pi/4$ & $\pi/2$ & $\pi/4$ & $-2\cos(\delta - 2\theta) + 2\cos(\delta + 2\theta) + 5$ \\
\bottomrule
\end{tabular}
\caption{Intensity expressions for different $\beta$, $\eta$, $\alpha$, and $\rho$ values.}
\label{table:intensity_expressions}
\end{table*}


==> tables/captured_measurements.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}clcc@{}} % Adjusts column spacing
\toprule
\textbf{Measurement} & \multicolumn{1}{c}{\textbf{$\eta$ values}} & \textbf{$\beta$ values} & \textbf{Intensity Expression} \\
\midrule
$I_1$ & 0 & $\pi/4$ & $I_b + I_a \cos \delta$ \\
$I_2$ & 0 & $-\pi/4$ & $I_b - I_a \cos \delta$ \\
$I_3$ & 0 & 0 & $I_b - I_a \sin \delta \sin 2 (\theta - \gamma)$ \\
$I_4$ & $\pi/4$ & 0 & $I_b + I_a \sin \delta \cos 2 (\theta - \gamma)$ \\
$I_5$ & $\pi/2$ & 0 & $I_b + I_a \sin \delta \sin 2 ( \theta - \gamma)$ \\
$I_6$ & $3\pi/4$ & 0 & $I_b - I_a \sin \delta \cos 2 ( \theta - \gamma) $ \\
\bottomrule
\end{tabular}
\caption{6-step phase shifting technique for obtaining stress parameters per ray: Intensity expressions for different $\eta$ and $\beta$ values.}
\label{table:intensity_expressions}
\end{table}


\begin{comment}
$I_1$ & 0 & $\pi/4$ & $I_b + I_a \cos \delta$ \\
$I_2$ & 0 & $-\pi/4$ & $I_b - I_a \cos \delta$ \\
$I_3$ & 0 & 0 & $I_b - I_a \sin \delta \sin 2\theta$ \\
$I_4$ & $\pi/4$ & 0 & $I_b + I_a \sin \delta \cos 2\theta$ \\
$I_5$ & $\pi/2$ & 0 & $I_b + I_a \sin \delta \sin 2\theta$ \\
$I_6$ & $3\pi/4$ & 0 & $I_b - I_a \sin \delta \cos 2\theta$ \\
\end{comment}

==> tables/captured_measurements_abcd.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}lcccr@{}} % Added a new column for rho
\toprule
 & \multicolumn{1}{c}{\textbf{$\beta_1$ }} & \textbf{$\beta_2$ } & \textbf{$\alpha_2$ } & Expression \\
\midrule
$I_0$    & $\nicefrac{\pi}{4}$ & $0$                    & $0$                  &   $ 1 - 2ac + 2bd $\\
$I_1$    & $\nicefrac{\pi}{4}$ & $0$                    & $\nicefrac{\pi }{4}$ &   $ 2b^2 + 2c^2 $\\
$I_2$    & $\nicefrac{\pi}{4}$ & $0$                    & $\nicefrac{\pi }{2}$ &   $ 1 + 2ac - 2bd $\\
$I_3$    & $\nicefrac{\pi}{4}$ & $0$                    & $\nicefrac{3\pi}{4}$ &   $ 2a^2 + 2d^2 $\\
$I_4$    & $\nicefrac{\pi}{4}$ & $\nicefrac{\pi}{4}$    & $0$                  &   $ 2a^2 + 2d^2 $\\
$I_5$    & $\nicefrac{\pi}{4}$ & $\nicefrac{\pi}{4}$    & $\nicefrac{\pi }{4}$ &   $ 1 + 2ab + 2cd $\\
$I_6$    & $\nicefrac{\pi}{4}$ & $\nicefrac{\pi}{4}$    & $\nicefrac{\pi }{2}$ &   $ 2b^2 + 2c^2 $\\
$I_7$    & $\nicefrac{\pi}{4}$ & $\nicefrac{\pi}{4}$    & $\nicefrac{3\pi}{4}$ &   $ 1 - 2ab -2cd $\\
$I_8$    & $\nicefrac{\pi}{2}$ & $0$                    & $0$                  &   $ 2c^2 + 2d^2  $\\
$I_9$    & $\nicefrac{\pi}{2}$ & $0$                    & $\nicefrac{\pi }{4}$ &   $ 1 + 2ac + 2bd    $\\
$I_{10}$ & $\nicefrac{\pi}{2}$ & $0$                    & $\nicefrac{\pi }{2}$ &   $ 2a^2 + 2b^2  $\\
$I_{11}$ & $\nicefrac{\pi}{2}$ & $0$                    & $\nicefrac{3\pi}{4}$ &   $ 1 - 2ac - 2bd  $\\
$I_{12}$ & $\nicefrac{\pi}{2}$ & $\nicefrac{\pi}{4}$     & $0$                  &   $ 1 - 2ac - 2bd  $\\
$I_{13}$ & $\nicefrac{\pi}{2}$ & $\nicefrac{\pi}{4}$     & $\nicefrac{\pi }{4}$ &   $ 1 + 2ad - 2bc $\\
$I_{14}$ & $\nicefrac{\pi}{2}$ & $\nicefrac{\pi}{4}$     & $\nicefrac{\pi }{2}$ &   $ 1 + 2ac + 2bd $\\
$I_{15}$ & $\nicefrac{\pi}{2}$ & $\nicefrac{\pi}{4}$     & $\nicefrac{3\pi}{4}$ &   $ 1 - 2ad + 2bc $\\

% $I_4$ & $\pi/2$ & $0$    & $\pi/4$ & $0.5 + 0.5 \sin \delta \sin 2 (\gamma + \theta)$ \\
% $I_5$ & $\pi/2$ & $0$    & $\pi/2$ & $0.5 - 0.5 \cos(\theta + \gamma) \cos(\theta - \gamma)$ \\
%      &         &        &         & $- 0.5 \sin(\theta - \gamma) \sin(\theta + \gamma) \cos \delta$ \\
\bottomrule
\end{tabular}
\caption{\textbf{Captured polariscope measurements as a function of Jones matrix elements.} Upon varying rotation angles of QWP1 ($\beta_1$),QWP2($\beta_2$) and LP2 ($\alpha_2$), we capture measurements that encode the constituents $a$, $b$, $c$ and $d$ of the equivalent Jones matrix $\mathbf{J}_\text{eq}$ which in turn depends on the underlying stress field.}
\label{table:intensity_abcd}
\end{table}

